Dynamic Structural Clustering Unleashed: Flexible Similarities, Versatile Updates and for All Parameters

We study structural clustering on graphs in dynamic scenarios, where the graphs can be updated by arbitrary insertions or deletions of edges/vertices. The goal is to efficiently compute structural clustering results for any clustering parameters $\epsilon$ and $\mu$ given on the fly, for arbitrary graph update patterns, and for all typical similarity measurements. Specifically, we adopt the idea of update affordability and propose an a-lot-simpler yet more efficient (both theoretically and practically) algorithm (than state of the art), named VD-STAR to handle graph updates. First, with a theoretical clustering result quality guarantee, VD-STAR can output high-quality clustering results with up to 99.9% accuracy. Second, our VD-STAR is easy to implement as it just needs to maintain certain sorted linked lists and hash tables, and hence, effectively enhances its deployment in practice. Third and most importantly, by careful analysis, VD-STAR improves the per-update time bound of the state-of-the-art from $O(\log^2 n)$ expected with certain update pattern assumption to $O(\log n)$ amortized in expectation without any update pattern assumption. We further design two variants of VD-STAR to enhance its empirical performance. Experimental results show that our algorithms consistently outperform the state-of-the-art competitors by up to 9,315 times in update time across nine real datasets.

==> algo-framework.tex <==
\begin{algorithm}
\caption{Algorithm Framework}\label{alg:framework}
\DontPrintSemicolon
\SetKwComment{Comment}{/* }{ */}

\SetKwBlock{update}{Update procedure}{end}
\SetKwFunction{esm}{EdgeSimilarityMaintenance}
\SetKwFunction{csm}{CoreStatusMaintenance}

\SetKwBlock{query}{Query procedure}{end}
\SetKwFunction{icv}{IdentifyCoreVertex}
\SetKwFunction{cse}{CollectSimilarEdge}

        
\update{
    \esm{}{
        
    }
    \;
    \csm{}{
    
    }
}

\query{
    $V_{cr} = \emptyset$\;
    $E_{cr} = \emptyset$\;
    Initiate an empty graph $G_{cr}$\;
    \;
    \icv{$\mu$, $\epsilon$, $V_{cr}$, $D$}{     
        \KwRet $V_{cr}$\;
    }
    \;
    \cse{$\epsilon$, $V_{cr}$, $E_{cr}$, $NO$}{
    
        \For{each $v \in V_{cr}$}{
            obtain the similar edges by scanning $NO[u]$ and add to $E_{cr}$\;
            }
    
        \KwRet $E_{cr}$\;
    }
    \;
    Add $V_{cr}$ and $E_{cr}$ to $G_{cr}$\;
    \KwRet Clustering results from $G_{cr}$ \;
}

\end{algorithm}

==> figures/figure_scripts/eta_varying_old.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.9\linewidth}
        \includegraphics[width=\textwidth]{figures/update_generation/lines_legend_ug.pdf}
    \end{subfigure}
    \begin{tabular}{ccc}
        \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
            \includegraphics[width=\textwidth]{figures/insertion_ratio/soc.pdf}
            \vspace{-6mm}
            \caption{Slash}
            \vspace{-2mm}
        \end{subfigure}&
            \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
                \includegraphics[width=\textwidth]{figures/insertion_ratio/NotreDame.pdf}
                \vspace{-6mm}
                \caption{ND}
                \vspace{-2mm}
        \end{subfigure}&
            \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
                \includegraphics[width=\textwidth]{figures/insertion_ratio/google.pdf}
                \vspace{-6mm}
                \caption{Google}
                \vspace{-2mm}
        \end{subfigure}\\
            \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
                \includegraphics[width=\textwidth]{figures/insertion_ratio/topcats.pdf}
                \vspace{-6mm}
                \caption{Topcats}
                \vspace{-2mm}
        \end{subfigure}&
            \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
                \includegraphics[width=\textwidth]{figures/insertion_ratio/pokec.pdf}
                \vspace{-6mm}
                \caption{Pokec}
                \vspace{-2mm}
        \end{subfigure}&
        \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
            \includegraphics[width=\textwidth]{figures/insertion_ratio/skitter.pdf}
            \vspace{-6mm}
            \caption{Skitter}
            \vspace{-2mm}
        \end{subfigure}\\
        \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
            \includegraphics[width=\textwidth]{figures/insertion_ratio/talk.pdf}
            \vspace{-6mm}
            \caption{Talk}
            \vspace{-2mm}
        \end{subfigure}&
        \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
            \includegraphics[width=\textwidth]{figures/insertion_ratio/orkut.pdf}
            \vspace{-6mm}
            \caption{Orkut}
            \vspace{-2mm}
        \end{subfigure}&
        \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
            \includegraphics[width=\textwidth]{figures/insertion_ratio/LiveJournal.pdf}
            \vspace{-6mm}
            \caption{LiveJournal}
            \vspace{-2mm}
        \end{subfigure}\\
    \end{tabular}
    \vspace{-3mm}
    \caption{Average update time vs. $\eta$}
    \label{fig:eta_varying}
\vspace{-6mm}
\end{figure}


==> figures/figure_scripts/rho_varying_old.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.7\linewidth}
        \includegraphics[width=\textwidth]{figures/rho_varying/lines_legend_rho.pdf}
    \end{subfigure}
    \begin{tabular}{ccc}
        \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
            \includegraphics[width=\textwidth]{figures/rho_varying/soc.pdf}
            \vspace{-6mm}
            \caption{Slash}
            \vspace{-2mm}
        \end{subfigure}&
            \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
                \includegraphics[width=\textwidth]{figures/rho_varying/NotreDame.pdf}
                \vspace{-6mm}
                \caption{ND}
                \vspace{-2mm}
        \end{subfigure}&
            \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
                \includegraphics[width=\textwidth]{figures/rho_varying/google.pdf}
                \vspace{-6mm}
                \caption{Google}
                \vspace{-2mm}
        \end{subfigure}\\
            \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
                \includegraphics[width=\textwidth]{figures/rho_varying/topcats.pdf}
                \vspace{-6mm}
                \caption{Topcats}
                \vspace{-2mm}
        \end{subfigure}&
            \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
                \includegraphics[width=\textwidth]{figures/rho_varying/pokec.pdf}
                \vspace{-6mm}
                \caption{Pokec}
                \vspace{-2mm}
        \end{subfigure}&
        \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
            \includegraphics[width=\textwidth]{figures/rho_varying/skitter.pdf}
            \vspace{-6mm}
            \caption{Skitter}
            \vspace{-2mm}
        \end{subfigure}\\
        \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
            \includegraphics[width=\textwidth]{figures/rho_varying/talk.pdf}
            \vspace{-6mm}
            \caption{Talk}
            \vspace{-2mm}
        \end{subfigure}&
        \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
            \includegraphics[width=\textwidth]{figures/rho_varying/orkut.pdf}
            \vspace{-6mm}
            \caption{Orkut}
            \vspace{-2mm}
        \end{subfigure}&
        \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
            \includegraphics[width=\textwidth]{figures/rho_varying/LiveJournal.pdf}
            \vspace{-6mm}
            \caption{LiveJournal}
            \vspace{-2mm}
        \end{subfigure}\\
    \end{tabular}
    \vspace{-3mm}
    \caption{Average update running time vs.  $\rho^*$}
    \label{fig:rho_varying}
\vspace{-3mm}
\end{figure}


==> figures/figure_scripts/update_generation_varying_old.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.9\linewidth}
        \includegraphics[width=\textwidth]{figures/update_generation/lines_legend_ug.pdf}
    \end{subfigure}
    \begin{tabular}{ccc}
        \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
            \includegraphics[width=\textwidth]{figures/update_generation/soc.pdf}
            \vspace{-8mm}
            \caption{Slash}
            \vspace{-2mm}
        \end{subfigure}&
            \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
                \includegraphics[width=\textwidth]{figures/update_generation/NotreDame.pdf}
                \vspace{-8mm}
                \caption{ND}
                \vspace{-2mm}
        \end{subfigure}&
            \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
                \includegraphics[width=\textwidth]{figures/update_generation/google.pdf}
                \vspace{-8mm}
                \caption{Google}
                \vspace{-2mm}
        \end{subfigure}\\
            \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
                \includegraphics[width=\textwidth]{figures/update_generation/topcats.pdf}
                \vspace{-8mm}
                \caption{Topcats}
                \vspace{-2mm}
        \end{subfigure}&
            \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
                \includegraphics[width=\textwidth]{figures/update_generation/pokec.pdf}
                \vspace{-8mm}
                \caption{Pokec}
                \vspace{-2mm}
        \end{subfigure}&
        \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
            \includegraphics[width=\textwidth]{figures/update_generation/skitter.pdf}
            \vspace{-8mm}
            \caption{Skitter}
            \vspace{-2mm}
        \end{subfigure}\\
        \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
            \includegraphics[width=\textwidth]{figures/update_generation/talk.pdf}
            \vspace{-8mm}
            \caption{Talk}
            \vspace{-2mm}
        \end{subfigure}&
        \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
            \includegraphics[width=\textwidth]{figures/update_generation/orkut.pdf}
            \vspace{-8mm}
            \caption{Orkut}
            \vspace{-2mm}
        \end{subfigure}&
        \hspace{-3mm}\begin{subfigure}{0.333\linewidth}
            \includegraphics[width=\textwidth]{figures/update_generation/LiveJournal.pdf}
            \vspace{-8mm}
            \caption{LiveJournal}
            \vspace{-2mm}
        \end{subfigure}\\
    \end{tabular}
    \vspace{-3mm}
    \caption{Average update time vs. update distribution}
    \label{fig:ug_varying}
\vspace{-4mm}
\end{figure}



==> sections/Related_work.tex <==
\section{Other Related Work}
\label{sec:rl}
The Structural Clustering problem was first proposed by Xu~\shortauthors~\cite{xu2007scan}, together with an algorithm named \emph{SCAN} based on \emph{breadth-first-search}. 
%<<<<<<< HEAD
The bottleneck of \emph{SCAN} is the similarity computation on each edge, and it has been shown that the overall time complexity of {\em SCAN} is $O(m^{1.5})$.
%where $d_{\max}$ is the largest degree in the graph and in the worst case, $d_{\max}$ can be as large as $n$. 
Follow-up studies~\cite{shiokawa2015scan++, chang2017mathsf} proposed heuristic methods to accelerate the computation. 
%=======
%The bottleneck of \emph{SCAN} is the similarity computation on each edge which takes an overall cost of $O(m \cdot d_{\max})$, where $d_{\max}$ is the largest degree in the graph -- in the worst case, $d_{\max}$ can be as large as $n$. 
%Follow-up studies~\cite{shiokawa2015scan++, chang2017mathsf} proposed heuristic algorithms to accelerate the computation. 
%>>>>>>> 9c543e8cabedcf54a6b007f39f5594713c74b73f
For instance, \emph{SCAN++}~\cite{shiokawa2015scan++} builds a two-hop neighbor-based structure, and \emph{pSCAN}~\cite{chang2017mathsf} prunes the vertices that are infeasible to become core vertices. 
However, these methods do not improve the worst-case time complexity. 
\emph{LinkSCAN*}~\cite{lim2014linkscan} applied a sampling-based method to accelerate the similarity computation without error bounds. 
In addition, its focus is on a transformed graph, where the edges become vertices. 

These algorithms all focus on static graphs. 
They become inefficient when there are updates to the graphs. When there is a graph update, i.e., an edge insertion or deletion $(u, v)$, it impacts all the neighbors of the two relevant vertices $u$ and $v$. 
As shown by a hard instance~\cite{ruan2021dynamic},
an $\Omega(d_{\max})$ time is inevitable for algorithms that maintain the edge labels (whether its two end-vertices are similar or dissimilar).
%
Another series of works~\cite{tseng2021parallel, che2018parallelizing, stovall2014gpuscan, zhao2013pscan, takahashi2017scan} focuses on parallelizing the algorithms, which are orthogonal to our work.
%Assuming that the maximum degree is $d$. Then, there are $O(d)$ neighboring vertices for which the similarity scores need to be recomputed. Each similarity score computation takes $O(d)$ time if it is done from scratch. The total update time is then $O(d^2)$. As $d$ can be as large as $n$, the number of vertices in the graph, the update time is $O(n^2)$ in the worst case.
%
% \vspace{1mm}
% \noindent\textbf{Dynamic structural clustering.}
% %To solve the problem in a dynamic scenario, 
% DynELM~\cite{ruan2021dynamic} presents an efficient structural clustering method for graphs with dynamic updates, through bounded approximation that allows a $\rho$  error in similarity estimation. Under a $\rho$-approximation bound, it proposes a sampling-based method to compute the clustering results, which reduces the similarity measurement time complexity from $O(n)$ to $O(\log n \log \frac{M}{p_f})$ with a high success rate of $1-p_f$, where $n = |V|$ and $M$ is the number of updates.  
% To accommodate graph updates, DynELM shows that an edge can afford $l$ affecting updates before it impacts the approximated clustering results. Here, an affecting update refers to an update capable of affecting the similarity measurement on the edge. 
% A \emph{distributed tracking} (DT)-based framework that tracks the number of updates affecting an edge is introduced, which helps achieve an amortized $O(\log^2 n + \log n \log \frac{M}{p_f})$ update time complexity. The sampling-based method, coupled with the DT framework, effectively reduces the update cost of the dynamical structural clustering problem while achieving high-quality results. Nonetheless, in their defined problem scope, the parameters $\epsilon$ and $\mu$ are predetermined, and they do not support result indexing.
%
% \vspace{1mm}
% \noindent\textbf{Index schema.}
% The GS*-Index~\cite{wen2017efficient} treats $\mu$ and $\epsilon$ as user-defined input parameters. It introduces an index schema to process structural clustering queries in time linear to the clustering result size for any given $\mu$ and $\epsilon$. Its core idea is to build a table with each row representing a possible $\mu$ value, which is detailed in Section~\ref{subsec:gs-index}. However, its drawback arises when dealing with graph updates, as updating the table takes $O(d^2)$ time, which could become prohibitively expensive for large graphs.
% When there is a graph update, GS*-Index takes $O(d^2)$ time to update the table, which could be too costly on large graphs. 
%
% Building upon DynELM and GS*-Index, BOTBIN~\cite{zhang2022effective} supports both result indexing and updates. It follows the $\rho$-approximation setting and applies a \emph{bottom-$k$ hashing} to estimate similarity scores.  Similar to GS*-Index, a table is built, and an average update time complexity of $O(\log n \log \frac{M + m}{p_f})$  is achieved, benefiting from its $\epsilon$-bucketing method for table size reduction and hashing for similarity measurement cost reduction. However, due to vertex ID permutation for hashing,  handling vertex insertions becomes non-trivial. When a new vertex is inserted, it must be shuffled into the previous vertex ID to maintain the hashing technique. This shuffling can change the bottom-$k$ results of the affected vertex's neighborhood, resulting in an $O(d)$ time cost to update the bottom-$k$ results. In addition, their claimed complexity may not always hold in certain update distributions. When an update $(u, w)$ comes, they assume that it has $\frac{k}{d_u}$ probability to change the bottom-$k$ result of $N[u]$ and to re-compute the similarity, hence a lower time complexity on average. This assumption holds only when the update is uniformly distributed, i.e., each vertex has an equal chance of being affected. 
% In real-world applications, frequent updates that could affect bottom-$k$ results might invalidate this probability claim.



==> sections/algo-update.tex <==
\begin{algorithm}
\caption{Our Implementation of {\em EdgeSimStr}.update}\label{algo:update}
%\DontPrintSemicolon
\SetKwComment{Comment}{/* }{ */}

\SetKwBlock{update}{Update Procedure:}{end}
\SetKwFunction{esm}{EdgeSimStr}
\SetKwFunction{esf}{EdgeSimStr.find}
\SetKwFunction{esu}{EdgeSimStr.update}
\SetKwFunction{esc}{EdgeSimStr.cal-sim}

\SetKwFunction{csu}{CoreFindStr.update}

\SetKwBlock{query}{Query Procedure:}{end}
\SetKwFunction{icv}{CoreFindStr.find-core}
%\SetKwFunction{cse}{CollectSimilarEdge}

        
\KwIn{either an insertion or a deletion of edge $(u,v)$} 
%indicated by  $op \in \{\text{insertion}
%, \text{deletion}\}$ }

$c_u \leftarrow c_u + 1$; $c_v \leftarrow c_v + 1$\;
\end{algorithm}


==> sections/backup-Methodology.tex <==
\section{Our Versatile DynStrClu Algorithm}
\label{sec:our-algo}

Next, we introduce our solution called {\em Versatile Dynamic Structural Clustering} ({\em Ver-DynStrClu}) which not only overcomes {\em all} the aforementioned limitations of BOTBIN, but also improves the per-update running time cost to $O(\log n + \log M)$ amortized in expectation. 

Without loss of generality, we assume that the number of updates $M$ is at most $n^2$, because, otherwise, we can rebuild everything from scratch in our {\em Ver-DynStrClu} in $O(n^2 \log n + m)$ expected time and hence, each of such $ M = n^2$ updates is charged a $O(\log n)$ expected amortized cost which does not affect the per-update running time bound.   
Moreover, as we shall see shortly, 
the randomness in the running time only comes from the use of hash tables.
%
In this and the next section, we prove the following theorem:
\begin{theorem}
Our {\em Ver-DynStrClu} algorithm supports all the three similarity measurements (Jaccard, Cosine, Dice).
It can return an $\rho$-absolute-approximate clustering result with high probability at least $1 - \frac{1}{n}$ for each query and can handle each update in $O(\log n)$ expected amortized time.  
The space consumption of {\em Ver-DynStrClu} is bounded by $O(n + m)$ at all times.
\end{theorem}

%\subsection{The {\em Ver-DynStrClu} Algorithm}

As mentioned earlier, our {\em Ver-DynStrClu} works under the unified algorithm framework (Algorithm~\ref{algo:framework}). 
As a result, we just need to consider the implementations of {\em Ver-DynStrClu} 
for the two data structures {\em CoreFindStr} and {\em EdgeSimStr}, respectively.
%
Specifically, our {\em Ver-DynStrClu} adopts the implementation of BOTBIN for {\em CoreFindStr}, i.e., the $\Delta$-table technique with $\Delta = \frac{1}{2} \rho$.
Therefore, in the remaining of this section, we focus on our implementation for {\em EdgeSimStr}.

%\subsection{The Implementaion for {\em EdgeSimStr}}

\subsection{Update Affordability and Background}

Our {\em Ver-DynStrClu} adopts the notion of $\rho$-absolute-approximation.
Thanks to this approximation notion, 
{\em Ver-DynStrClu} is allowed to just maintain {\em approximate} rather than exact similarities, 
%within an $\rho$ absolute error, rather than exact similarities.
and thus, 
it creates rooms for efficiency improvements.
First, the similarity can now be estimated (within an $\rho$-absolute error) via certain sampling techniques efficiently.
Second, each edge can now afford certain number of affecting updates before its estimated similarity running outside of the $\rho$-absolute-error range since the last estimation.
Such a number of affecting updates is called the {\em update affordability} of the edge. 

\begin{definition}[Update Affordability]
\label{def:update-affordability}
For any edge $(u,v)$, 
consider the moment when an $\rho$-absolute-approximate similarity $\tilde{\sigma}(u,v)$ is just computed;
the {\em update affordability} of $(u,v)$ is 
%since then, 
the {\em minimum} number of 
affecting updates, denoted by $\tau(u,v)$,
%such that 
%it requires at least $\tau(u,v) \in \Omega(d_{\max}(u,v))$ affecting updates 
to make 
$\tilde{\sigma}(u,v)$ become {\em invalid}, in the sense that $|\tilde{\sigma}(u,v) - \sigma(u,v)| > \rho$.
%where $d_{\max}(u,v) = \max\{d_u, d_v\}$.
%and $0 \leq \rho \leq 1$ is a constant.  
\end{definition}

In fact, 
%these two observations were
the concept of the update affordability was first proposed and 
exploited by Ruan~\shortauthors~in~\cite{ruan2021dynamic} for solving {\em DynStrClu} problem for Jaccard similarity  with {\em pre-specified and fixed} parameters $\eps$ and $\mu$. 
We borrow this concept and extend it to {\em DynStrClu-AllPara} problem for {\em versatile} similarity measurements (Jaccard, Cosine, and Dice).
As we showed in Section~\ref{sec:update-affordability}, 
the extension of the concept of update affordability from Jaccard to Cosine similarity is challenging and non-trivial, because of the {\em non-linear} denominator (that is, $\sqrt{n_u\cdot n_v}$) in the Cosine similarity measurement.

To avoid distraction,
we defer the proof of the following claim to Section~\ref{sec:update-affordability}.

\begin{claim}
\label{claim:update-affordability}
For any edge $(u,v)$, 
the update affordability $\tau(u,v) \in \Omega(d_{\max}(u,v))$ holds for any of Jaccard, Cosine and Dice similarity measurements,
%consider the moment when an $\rho$-absolute-approximate (either Jaccard, Cosine or Dice) similarity $\tilde{\sigma}(u,v)$ is just computed;
%since then, it requires at least $\tau(u,v) \in \Omega(d_{\max}(u,v))$ affecting updates 
%to make $\tilde{\sigma}(u,v)$ become {\em invalid}, in the sense that $|\tilde{\sigma}(u,v) - \sigma(u,v)| > \rho$, 
where $d_{\max}(u,v) = \max\{d_u, d_v\}$.
%and $0 \leq \rho \leq 1$ is a constant.  
\end{claim}
%
%The value $\tau(u,v)$ in Claim~\ref{claim:update-affordability} is called the {\em update affordability} of edge $(u,v)$. 
By definition of the update affordability,
when an approximate similarity $\tilde{\sigma}(u,v)$ of an edge $(u,v)$ is just computed,
$\tilde{\sigma}(u,v)$ will remain valid for the next $\tau(u,v)-1$ affecting updates.
And hence, 
in order to maintain a valid $\rho$-absolute-approximate similarity for every edge in the graph, one has to re-compute $\tilde{\sigma}(u,v)$ no later than the $\tau(u,v)^\text{th}$ affecting update for each $(u,v) \in E$. 

However, observe that (i) the update affordability can be different for different edges, and 
(ii) an update of edge $(u,v)$
would ``consume'' one affordability for each of its $d_u + d_v \in O(d_{\max})$ affected edges.
Therefore, simply tracking the ``remaining'' update affordability for each affected edge for each affecting update  would lead to a running time cost of $\Omega(d_{\max})$ which is prohibitively expensive.
Therefore, it is challenging to identify the set $F$ of all invalid edges when an update arrives, without touching each of the affected edges.

%<<<<<<< HEAD
%Ruan~\shortauthors~\cite{} overcome this technical challenge for Jaccard similarity by adopting the {\em Distributed Tracking} technique~\cite{} to track the {\em exact moment} when the $\tau(u,v)^\text{th}$ affecting update arrives for each edge. 
%=======
Ruan~\shortauthors~\cite{ruan2021dynamic} overcome this technical challenge for Jaccard similarity by adopting the {\em Distributed Tracking} technique~\cite{} to track the {\em exact moment} when the $\tau(u,v)^\text{th}$ affecting update for each edge. 
%>>>>>>> e0f23dbf30678b7adb3223732f055e1c986d403d
They proved that their algorithm can achieve a $O(\log^2 n)$ amortized cost for identifying the set $F$ of invalid edges for each update.
%
Next, we show a simpler yet more efficient solution which identifies 
the invalid edge set $F$ just in $O(1)$ amortized time for each update.

\subsection{Our Implementation of {\em EdgeSimStr}}

%In order to identify the set $F$ of invalid affected edges,
%we propose a new solution called {\em Regular Edge }
\noindent
{\bf Rationale of Our Approach.}
The basic idea of our solution for identifying invalid edges is as follows.
For each edge $(u,v) \in E$, once $\tilde{\sigma}(u,v)$ is just computed, then compute 
its update affordability $\tau(u,v)$.
Instead of tracking the exact moment when the $\tau(u,v)^\text{th}$ affecting update arrives,
our algorithm aims to just identify an {\em arbitrary} moment when there are at least $\frac{1}{4} \lfloor \tau(u,v) \rfloor_2$ affecting updates happened, where $\lfloor \tau(u,v) \rfloor_2$ is the {\em largest power-of-two} integer that is no more than $\tau(u,v)$, namely, $\lfloor \tau(u,v) \rfloor_2 = 2^{\lfloor \log_2 \tau(u,v) \rfloor}$. 
And such a moment is called a {\em checkpoint moment} of edge $(u,v)$.
%
Clearly, $\lfloor \tau(u,v) \rfloor_2 \geq \frac{1}{2} \tau(u,v)$.
When a checkpoint moment of $(u,v)$ is identified, there must have been at least $\frac{1}{8} \tau(u,v) \in \Omega(\tau(u,v))$ affecting updates happened, which, as we shall see shortly, is sufficiently ``good enough'' for our theoretical analysis.

To capture the checkpoint moments, 
our algorithm, for each edge $(u,v)$, allocates an {\em affordability quota}, denoted by $q(u,v) = \frac{1}{4}\lfloor \tau(u,v) \rfloor_2$, to the vertices $u$ and $v$.
Once 
%a checkpoint moment of $(u,v)$ is identified,
an arbitrary moment when the number of affecting updates incident on either $u$ or $v$ since the quota is allocated is $\geq q(u,v)$ is observed,
$(u,v)$ is then reported as an invalid edge.
%whose approximate similarity $\tilde{\sigma}(u,v)$ is re-computed. 
%and tracks the number of affecting updates incident on $u$ (and that on $v$, separately) since the quota is allocated.
The challenge is how to capture a checkpoint moment for each edge $(u,v)$ before its $\rho$-absolute-approximate $\tilde{\sigma}(u,v)$ becomes invalid, without touching all of the affected edges for every affecting update. 

\vspace{1mm}
\noindent
{\bf The Data Structure for {\em EdgeSimStr}.}
For each vertext $u\in V$, our {\em Ver-DynStrClu} maintains the following information for {\em EdgeSimStr} in the unified algorithm framework (Algorithm~\ref{algo:framework}):
\begin{itemize}[leftmargin = *]
\item a counter $c_u$ which records the number of affecting updates incident on $u$ up to date;
initially, $c_u \leftarrow 0$;
\item a {\em sorted bucket linked list} $\mathcal{B}(u)$, where:
\begin{itemize}
\item each bucket $B_i$ corresponds to a {\em unique index} $i$ (for $0 \leq i \leq \lceil \log_2 n \rceil$);
%and corresponds to the group of $u$'s neighbors with a quota of $2^i$;
\item bucket $B_i$ stores all the neigbors $w \in N(u)$ such that the affordability quota  $q(u, w) = 2^i$;
%moreover, each neighbor $v \in B_i(u)$ is stored along with two auxiliary information:
%\begin{itemize}
%\item a {\em checkin counter} $\bar{c}_u(v)$ which records the counter value $c_u$ of $u$ when $v$ is inserted to $B_i(u)$;
%\item a {\em flag} $isVisited$ which indicates whether $v$ has been visited once in $B_i(u)$;  
%\end{itemize} 
\item all the {\em non-empty} buckets $B_i$ which contains at least one neighbor $w \in N(u)$ are materialized in the sorted linked list $\mathcal{B}(u)$ in an {\em increasing order} by their indices $i$. 
\item each non-empty bucket $B_i \in \mathcal{B}(u)$ maintains a counter $\bar{c}_u(B_i)$ which records the counter value $c_u$ of $u$ when $B_i$ is last visited; initially, $\bar{c}_u(B_i)$ is set as the value of $c_u$ when $B_i$ is materialized and added to $\mathcal{B}(u)$; 
\end{itemize} 
\end{itemize}

\begin{comment}
\begin{fact}[\cite{zhuo's rts paper}]\label{fact:sorted-linked-list}
The sorted linked list $\mathcal{B}(u)$ can be maintained with $O(|\mathcal{B}(u)|)$ space and support the following in $O(1)$ expected time: 
\begin{itemize}[leftmargin = *]
\item an insertion or deletion of a bucket to or from $\mathcal{B}(u)$, and  
%can be performed in $O(1)$ expected time, and 
\item return the pointer of 
%the {\em predecessor bucket} $B_i$ of $B_j$ 
%in $\mathcal{B}(u)$ 
%can found in $O(1)$ expected time 
%such that $B_i$ is 
the largest bucket $B_i \in \mathcal{B}(u)$ with index $i \leq j$, for 
%$B_i \in \mathcal{B}(u)$ can be returned  
any given integer index $0 \leq j \leq \lceil \log_2 n \rceil$. 
\end{itemize}
\end{fact}

\begin{lemma}
The overall space consumption of the implementation of {\em Ver-DynStrClu} for {\em EdgeSimStr} is bounded by $O(n + m)$. 
\end{lemma}
\begin{proof}
Since $\mathcal{B}(u)$ stores non-empty buckets only, thus $|\mathcal{B}(u)| \leq d_u$ for each vertex $u\in V$. 
Combining Fact~\ref{fact:sorted-linked-list} and summing over all $u$'s, 
the overall space consumption is bounded by $O(n + m)$. 
\end{proof}
\end{comment}


\noindent
{\bf Implementation of {\em EdgeSimStr}.update($(u,v)$, $op$).}
In our {\em Ver-DynStrClu}, the update function of {\em EdgeSimStr} just increases
the counters $c_u$ and $c_v$ by one, respectively, i.e.,
$c_u \leftarrow c_u +1$ and $c_v \leftarrow c_v + 1$, 
recording that there is one more affecting update on them.

\vspace{1mm}
\noindent
{\bf Implementation of {\em EdgeSimStr}.insert($(u,v)$).}
The detailed implementation of the insert function is shown in Algorithm~\ref{algo:insert}.
To insert an edge $(u,v)$ to {\em EdgeSimStr}, 
our algorithm first compute the affordability quota $q(u,v)$ with the newly computed $\tilde{\sigma}(u,v)$, 
and then inserts $v$ (resp., $u$) to a proper bucket in $\mathcal{B}(u)$ (resp., $\mathcal{B}(v)$).
If the bucket does not exist, then create the bucket and insert it to the sorted bucket linked list accordingly.


\input{sections/algo-insert}

\vspace{1mm}
\noindent
{\bf Implementation of {\em EdgeSimStr}.delete($(u,v)$).}
This function just removes $v$ (resp., $u$) from its corresponding bucket in $\mathcal{B}(u)$ (resp., $\mathcal{B}(v)$. If the bucket becomes empty, then remove the bucket from the bucket list accordingly.
The pseudo code is shown in Algorithm~\ref{algo:delete}.

\input{sections/algo-delete}

\vspace{1mm}
\noindent
{\bf Implementation of {\em EdgeSimStr}.find($(u,v)$, $op$).}
Algorithm~\ref{algo:find} give the pseudo code of our implementation.
Observe that all the neighbors $w$ of $u$ are stored in a sorted list of {\em power-of-two} buckets of their corresponding affordability quotas.
When the counter $c_u$ is increased by one, 
it suffices to scan the sorted bucket list to check all the non-empty buckets $B_i$ such that 
the current $c_u$ has passed across (again) of their corresponding power-of-two values $2^i$ since they were last visited when $c_u = \bar{c}_u(B_i)$, see Line~4 in Algorithm~\ref{algo:find}.
For each of such buckets $B_i$,
our algorithm reports and adds the edge $(u,w)$ to $F$ for each $w \in B_i$ such that 
$w$ is visited in $B_i$ for the {\em second time}.
Perform the same process for $v$ symmetrically. 
The correctness of this implementation is proved in Section~\ref{sec:correctness}.
%The main idea of Algorithm~\ref{algo:find} is that 


%when the counter $c_u$ is increased by one, 

\input{sections/algo-find}

%<<<<<<< HEAD
\vspace{1mm}
\noindent
{\bf Implementation of {\em EdgeSimStr}.cal-sim($(x,y)$).}
See the detailed steps in Algorithm~\ref{algo:calsim}.

\input{sections/algo-calsim}

\subsection{The Overall {\em Ver-DynStrClu} Algorithm}

Substituting our implementation of {\em EdgeSimStr} and the $\Delta$-table implementation for {\em CoreFindStr} to the Unified Algorithm Framework (Algorithm~\ref{algo:framework}) gives the overall implementation of our {\em Ver-DynStrClu} algorithm.

\section{old version}
%=======
\subsection{A Similarity Estimator}
We first propose a sampling-based method for estimating the similarity.
%>>>>>>> e0f23dbf30678b7adb3223732f055e1c986d403d

Consider an arbitrary edge $(u,v)$; let $a = |N[u]\cap N[v]|$, $b_1 = |N[u]|$, and $b_2 = |N[v]|$. Without losing the generality, we assume $b_2$ is not smaller than $b_1$. We define a random variable $X$ which is generated by the following steps:
\begin{enumerate}
    \item Draw a vertex $w$ from $N[v]$ uniformly at random.  
    \item Check if $w \in N[u]$, if so, $X=1$; otherwise $X=0$.
\end{enumerate}
From the procedures, we have $Pr[X=1] = \frac{a}{b_2}$.
Let $X_1, X_2, ... X_L  $ be $L$ independent instances of the random variable $X$, and define $\Bar{X} = \frac{1}{L}\sum_{i=1}^LX_i$, and we can get $E[\Bar{X}] = \frac{a}{b_2}$. Hence, 
\begin{itemize}
\item {\em Jaccard similarity}: 
$\sigma(u,v) = \frac{b_2E[\Bar{X}]}{b_1 + b_2 - b_2E[\Bar{X}]}$
\item {\em Cosine similarity}: 
$\sigma(u,v) = \frac{a}{\sqrt{b_1 \cdot b_2}} = \sqrt{\frac{b_2}{b_1}}E[\Bar{X}]$
\item {\em Dice similarity}: 
$\sigma(u,v) = \frac{b_2E[\Bar{X}]}{(b_1 + b_2)/2}$.
\end{itemize}
\subsubsection{Jaccard Similarity}
\begin{theorem}
    Define $\tilde{\sigma}(u,v) = \frac{b_2\Bar{X}}{b_1 + b_2 - b_2\Bar{X}}$. By setting $L = $, we have $\mathbf{Pr}[|\tilde{\sigma}(u,v) - \sigma(u,v)| > \rho] \leq p$.
\end{theorem}
\begin{proof}
    $\mathbf{Pr}[|\tilde{\sigma}(u,v) - \sigma(u,v)| > \rho] = \mathbf{Pr}[|\frac{b_2E[\Bar{X}]}{b_1 + b_2 - b_2E[\Bar{X}]} - \frac{b_2\Bar{X}}{b_1 + b_2 - b_2\Bar{X}}| > \rho] = \mathbf{Pr}[\frac{(b1b_2+b_2^2)(|\Bar{X} - E[\Bar{X}]|}{(b_1 + b_2 - b_2E[\Bar{X}])((b_1 + b_2 - b_2\Bar{X})} > \rho]$
\end{proof}

\subsubsection{Cosine similarity}
We now prove that, with this sampling method, we can estimate the similarity in $O(\log\frac{2}{p})$ time. We consider the estimation in two cases:

(1) When $\min(d_u,d_v) < \epsilon^2\max(d_u,d_v)$, we can instantly label $u$ and $v$ as dissimilar, as $\sigma_c(u,v) = \frac{|N[u]\cap N[u]|}{\sqrt{d_u\cdot d_v}} < \frac{\min(d_u, d_v)}{\sqrt{d_u\cdot d_v}} <  \frac{\min(d_u, d_v)}{\sqrt{\frac{1}{\epsilon^2}\min(d_u, d_v)^2}} = \epsilon$. 

(2) When $\min(d_u,d_v) \geq \epsilon^2\max(d_u,d_v)$, we would like to compute the probability when the estimated similarity is out of the error bound, that is: 
$$Pr[|\Tilde{\sigma}(u,v) -\sigma(u,v)| > \rho]$$
Substitute with $\Bar{X}$, and we have:
$$Pr[\sqrt{\frac{b_2}{b_1}}|\Bar{X} - E[\Bar{X}]| > \rho]$$
As $\min(d_u,d_v) \geq \epsilon^2\max(d_u,d_v) \rightarrow \sqrt{\frac{b_2}{b_1}} \leq \frac{1}{\epsilon}$, we can get:
$$Pr[\sqrt{\frac{b_2}{b_1}}|\Bar{X} - E[\Bar{X}]| > \rho] \leq Pr[|\Bar{X} - E[\Bar{X}]| > \rho\epsilon]=p$$ 
By Hoeffding bound~\cite{hoeffding1994probability}, when the sample size $k = \frac{2}{\epsilon^2\rho^2}\ln{\frac{2}{p}}$, we have $Pr[|\Tilde{\sigma(u,v)} - \sigma(u,v)| > \rho] ]\leq p$. 

However, the deduced $k$ is related to $\epsilon$ which is an input parameter. To remove $\epsilon$ dependency from $k$, we discuss two cases:

(1) When $\epsilon \leq \rho$, we instantly get the clustering result as all edges can be labeled as similar due to $\sigma(u,v) > \epsilon - \rho $. 

(2) When $\epsilon > \rho$, it is safe to select $k = \frac{2}{\rho^4}\ln{\frac{2}{p}}$ which is not smaller than $\frac{2}{\epsilon^2\rho^2}\ln{\frac{2}{p}}$. 

As we need to sample twice in each neighbor, the time complexity is $O(2k) = \frac{4}{\rho^4}\ln{\frac{2}{p}} \in O(\log\frac{2}{p})$ that is the same as Jaccard Similarity.








\section{Proposed Method}
\label{sec:method}
\noindent\textbf{An Overview}.~To address the limitations mentioned earlier, we introduce our \algo~algorithm, which achieves an amortized update cost of $O(\log n)$ and supports all three similarity measures as well as new vertex insertions without relying on any update pattern assumptions. Our algorithm follows the same framework of DynELM~\cite{ruan2021dynamic} regarding graph updates (as described in Section~\ref{subsec:rho}), i.e., we only recalculate the similarity of an edge when its affordability runs out. However, instead of maintaining labels of the edges, we maintain a sorted linked list ($NO$) for each vertex neighborhood sorted by the similarity between neighbors and the vertex. This allows us to support on-the-fly parameter queries as described in Section~\ref{sec:preli}. While using the same framework, we propose a novel method to track the update affordability, improving the complexity from $O(\log^2 n)$ to $O(1)$ amortized. With this improvement, the bottleneck of our algorithm becomes maintaining the sorted linked list which has a lower bound $\Omega(\log n)$. Therefore, the complexity of our algorithm ($O(\log n)$) is optimal for this problem. 
%
Additionally, with the optimization methods that will be detailed in Secton~\ref{sec:opt}, our method can achieve $O(n_{cr} + m_{cr})$ query time for on-the-fly parameter queries.

In this section, we will describe our methods under the Jaccard similarity measure for easier presentation and we will expand it to other similarity measures in Section~\ref{subsec:cos}. We use the same sampling method introduced in~\cite{ruan2021dynamic}, and will focus on our novel method (regular similarity check) to track the update affordability, followed by the description of our schema supporting on-the-fly parameters and theoretical analysis. 


\subsection{Similarity Estimation}
% \label{subsubsec:se}
% We first present our algorithm using Jaccard similarity, which will be extended to cosine similarity later. For Jaccard similarity, we can apply the sampling method~\cite{ruan2021dynamic} to compute $\sigma(u,v)$. Consider an edge $(u ,v)$, the sampling method first generates a variable $X$ in the following steps:
% \begin{itemize}
%     \item Flip a coin with probability $\frac{|N[u]|}{|N[u]| + |N[v]|}$ to be 1, and with probability $\frac{|N[v]|}{|N[u]| + |N[v]|}$ to be 0.
%     \item If the result of the coin is 1, randomly pick a vertex from $N[u]$, otherwise, randomly pick a vertex from $N[v]$.
%     \item check if the picked vertex is in $N[u]\cap N[u]$; if it is, $X = 1$, otherwise $X = 0$.
% \end{itemize}
% The estimated similarity $\hat{\sigma}(u,v)$ can then be calculated as $\frac{\Bar{X}}{2-\Bar{X}}$, where $\Bar{X}$ is the expectation value of $k$ independent instances of $X$. Deduced from the Hoeffding inequality~\cite{hoeffding1994probability}, they further prove that: 

\begin{fact}[\cite{ruan2021dynamic}]
    There exists a sampling-based algorithm that can estimate the Jaccard similarity between two vertices satisfying $\rho$ approximation with $1 - p$ success rate when the sample size $k \geq \frac{2}{\rho^2}\ln{\frac{2}{p}} \in O(\log \frac{2}{p})$.
\end{fact}

For the $i^{th}$ estimation of a node pair, $p_i$ is set as $\frac{p_f}{i(i+1)}$ to ensure the $1-p_f$ success rate based on the Union Bound. The sample size of the $M^{th}$ estimation can then be bounded by $O(\log\frac{M}{p_f})$, and $\sigma(u,v)$ is bounded by expected $O(\log\frac{M}{p_f})$ with a hashing-based implementation to check if a vertex is in a set. 

\subsection{Regular Similarity Check}
\label{subsubsec:rscm}
We observe that it is unnecessary to recalculate similarity precisely when the edge undergoes $l$ updates. Instead, we can defer the recalculation until a significantly large number of updates have occurred, as long as the structural clustering results remain unchanged.  In pursuit of this more flexible update scheme, we introduce an effective module, namely the \emph{regular similarity check module (RSCM)}. Through a bucketing technique, our \emph{RSCM} significantly enhances the amortized time required for tracking the affected updates to $O(1)$.

\emph{RSCM} assigns a counter $s_u$ to each vertex $u$ that counts the number of updates on the vertex. For example, an insertion update $(u, w)$ will increase $s_u$ and $s_w$ by $1$. For each edge $(u, v)$, we assign a variable $\hat{c}_u(u, v)$ to record when we have (re-)computed $\sigma(u,v)$ and a threshold $th(u,v)$ that indicates when we should re-compute $\sigma(u,v)$, i.e., $\sigma(u,v)$ will be re-computed when $s_u = \hat{c}_u(u,v) + th(u,v)$. 

\begin{lemma}
    \label{lemma:threshold}
    When $th(u, v) = 2^{\lfloor\log_2{\frac{1}{4}\rho\max(d_u,d_v)\rfloor}}$, $\sigma(u,v)$ is re-computed before an edge $(u, v)$ changes from dissimilar to similar, or vice versa. 
\end{lemma}

\begin{proof}
    For an edge $(u, v)$, when $\sigma(u,v)$ is re-computed, there are at most $th(u, v) + th(v, u) - 1 \leq \lfloor\frac{1}{2}\rho\max(d_u,d_v)\rfloor$ updates affecting the edge. This is because only one of the counters has reached the threshold, and the other could have at least one update away from the threshold. With Fact~\ref{fact:flip}, Lemma~\ref{lemma:threshold} holds.
\end{proof}

\noindent\textbf{Bucketing technique.} To further enhance the efficiency of our \emph{RSCM}, we introduce a bucketing technique that groups the $th$ values of each vertex in buckets. Following the principles of Lemma~\ref{lemma:threshold}, $th$ values are written in the form of $2^i$, where $i$ is a positive integer greater than 1. For each vertex $u$, a linked list of buckets denoted as $L(u)$ is used. Each bucket is denoted as $B_i$ where $th(B_i)=2^i$ to store threshold values $th = 2^i$. Within each bucket, there exists a counter $\bar{s}_u(B_i)$ that records the shared counter value $s_u$ when elements in $B$ are re-computed. To reduce space usage and scanning time complexity, we store only the none-empty buckets in $L[u]$, sorted by the threshold size.

Next, we describe the process of our \emph{RSCM} algorithm to handle insertions and increase in $s_u$ values. 
 \begin{itemize}[leftmargin=*]
     \item Handling insertions: When a new edge $(u, v)$ is inserted, we calculate its $th$ and locate the bucket with the $th$ size. We create a bucket if it does not exist and set $\bar{s}_u(B_i) = s_u$. Then, we insert $\hat{c}_u(u, v) = s_u$ into the bucket.
     \item Handling increase in $s_u$: When the counter $s_u$ increases, we scan $L[u]$ and check whether $\lfloor\frac{s_u}{th(B)}\rfloor >  \lfloor\frac{s_u(B)}{th(B)}\rfloor$. If so, we update $\bar{s}_u(B)$ and examine the elements in the bucket. Otherwise, we can stop the scan as the later bucket has not reached its threshold. For the elements checked, we re-compute the similarity scores of the corresponding edges, calculate the new thresholds, and re-insert them into the new buckets.
 \end{itemize} 

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/bucket_RSCM.pdf}
    \caption{A running example of our bucketing technique}
    \label{fig:bucket_RSCM}
\end{figure}

%\noindent\textbf{A running example.} 
\begin{example}
Figure~\ref{fig:bucket_RSCM} shows a running example of our bucketing technique. When there is an update $(u, v)$, the counter $s_u$ is increased from 15 to 16. We first scan $B_2$. As $\lfloor\frac{16}{4}\rfloor > \lfloor\frac{12}{4}\rfloor$, we re-compute the similarity scores of $(u,v_3)$ and $(u,v_4)$. After that, we calculate their new thresholds, which are 4 and 16, respectively, and hence $\hat{c}(u,v_3)$ is inserted back into $B_2$, while $\hat{c}(u,v_4)$ is inserted into $B_4$ ($B_4$ is created as it did not exist before). Next, we scan $B_3$. Since $\lfloor\frac{16}{8}\rfloor > \lfloor\frac{8}{8}\rfloor$, similarly, $\sigma(u, v_2)$ is re-computed, and $\hat{c}(u,v_4)$ is inserted into $B_2$. We remove $B_3$ as it becomes empty. The algorithm stops at $B_4$ as $\lfloor\frac{16}{16}\rfloor = \lfloor\frac{16}{16}\rfloor$.
\end{example}


\noindent\textbf{Complexity analysis.} We now analyse the complexity of \emph{RSCM}.

\begin{lemma}
    \label{lemma:rscm}
    The running time of \emph{RSCM} is bounded by  $O(1)$ amortized.
\end{lemma}


\begin{fact}[\cite{zhangapproximate}]
\label{fact:bit_array}
    There exists an implementation that can find the successor bucket in $L[u]$ for any given $th$ in $O(1)$ amortized expected time with $O(|L(u)|)$ space. 
\end{fact}

\begin{proof}
\noindent\underline{Handling insertions.} Based on Fact~\ref{fact:bit_array}, locating the target bucket can be done in $O(1)$ amortized time. As $L[u]$ is a linked list, once the target bucket's successor is located, the cost of creating a new bucket is bounded by $O(1)$.

\noindent\underline{Handling increases in $s_u$.} When $s_u$ increases by 1, if there are $h_u$ buckets that have reached their threshold, the number of buckets scanned is $h_u + 1$. This is because our algorithm stops the scan right at the time when $\lfloor\frac{s_u}{th(B)}\rfloor >  \lfloor\frac{s_u(B)}{th(B)}\rfloor$ does not hold. The $O(1)$ time can be charged into the counter incremental cost (i.e., $s_u = s_u + 1$). For the $h_u$ buckets checked, as each bucket takes $th$ increases to reach the threshold, the $O(h_u)$ time cost can be charged into $th$ increases. Therefore, the amortized time cost of handling increases in $s_u$  is bounded by $O(1)$.
\end{proof}

\subsection{Dynamic Clustering for All Parameters}\label{subsec:for_all_p}
We now introduce how our algorithm can support the index schema to respond to queries for any $\epsilon$ and $\mu$ under our \emph{RSCM} framework. We first introduce an index schema capable of querying structural clustering results in $O(\mu n+m_{cr})$ time. This is followed by an outline of the primary steps of our algorithm, which accommodate graph updates, along with a theoretical analysis covering querying, updating, and space complexity. Additionally, we discuss how cosine similarity is accommodated within the index schema. In Section~\ref{sec:opt}, we will discuss variants of the index structure that support $O(n_{cr}+m_{cr})$ query. 

\subsubsection{Main Steps of Our Algorithm}
To query the structural clustering results in $O(\mu n+m_{cr})$ with any given $\mu$ and $\epsilon$, we maintain the sorted neighborhood, $NO[u]$, in a sorted linked list for each $u \in V$. We use a self-balancing binary search tree, denoted by $TO[u]$, to handle the sorting order of $NO[u]$ where the similarity scores are the key. Thus, the cost of each operation, e.g., a vertex insertion or deletion, can be bounded by $O(\log d_u)$.

Now, we describe the steps of our algorithm for index maintenance given a graph update $(u,v)$.
\begin{enumerate}[leftmargin=*]
    \item \textbf{Step 1.} Increase $s_u$ and $s_v$ by 1.
    \item \textbf{Step 2.}
    \begin{enumerate}[leftmargin=*]
        \item For inserting $(u, v)$,  calculate $\sigma (u,v)$ and insert $v$ into $NO[u]$, and create $th(u, v)$ in \emph{RSCM}.
        \item For deleting $(u, v)$, remove $v$ from $NO[u]$, and remove $th(u, v)$ in \emph{RSCM}.
    \end{enumerate}
    \item \textbf{Step 3.} Scan $L(u)$ and check whether any buckets  have reached their thresholds. Process the elements in those buckets following the procedure in Section~\ref{subsubsec:rscm}.
    \item \textbf{Step 4.} Perform a symmetric process of Steps 2 and 3 for $v$.
\end{enumerate}
 

\subsubsection{Theoretical Results}
\label{subsubsec:theory_analysis}
We prove the following theoretical results:
\begin{theorem}
    Given an approximation factor $\rho$ and a failure rate $p_f$, our algorithm 
    \begin{itemize}
        \item computes $G_C$ in $O(\mu n + m_{cr})$ time for any given $\epsilon$ and $\mu$;
        \item processes graph updates in $O(\log n + \log\frac{M}{p_f})$ amortized time; 
        \item computes similar edges  under the  $\rho$-approximation setting with at least $1 - p_f$ success probability.
    \end{itemize}
\end{theorem}

\noindent\textbf{Query time.} When inputting a pair of $\epsilon$ and $\mu$, for each vertex in $G$, we scan at most $\mu$ neighbors in $NO$ to decide whether the vertex is a core vertex. This is because $NO$ is a sorted list, and if the $\mu^{th}$ neighbor of a vertex has a similarity score smaller than $\epsilon$, the vertex cannot be a core vertex, otherwise, it is a core vertex. This process is bounded by $O(\mu n)$ time. For each core vertex, we continue with scanning $NO$ until we find the first neighbor whose similarity score is smaller than $\epsilon$. The scanned neighbors except for the last one are similar neighbors of the core vertex. This can be done within a BFS to output the clustering results. The whole process is bounded by $O(\mu n + m_{cr})$ time as the core vertex size is bounded by $n$. In real-world applications, $\mu$ is usually much smaller than $n$, e.g. 5 vs 10 million, which can be considered as a constant. In those cases, the complexity becomes $O(n + m_{cr})$. 

\noindent\textbf{Amortized update time.} Step 1 can be done in $O(1)$ time. For Step 2, computing $\sigma (u,v)$ is bounded by $O(\log\frac{M+m}{p_f})$ time expected as described in Section~\ref{subsubsec:rscm} ($m$ edges from sketch with $M$ updates). By using a binary search tree to maintain $NO$, each operation can be bounded by $O(\log n)$ time. For step 3,  with Lemma~\ref{lemma:rscm}, our \emph{RSCM} is bounded by $O(1)$ time amortized. For each $w \in N[u]$, we only re-compute the similarity score after it is affected for at least $th(u, w) \geq \frac{1}{8}\rho\max(d_u, d_w) = O(\max(d_u, d_w))$ times. Let $th^*$ be the smallest $th$ in $L[u]$, $d_u'$ be the degree of $u$ when $L[u]$ was created, we can get $d_u \leq d_u' + th^* \leq \frac{th^*}{\rho/2} + th^* = O(1)\cdot th^*$ as there are at most $th^*$ edge insertions to $u$; otherwise, the corresponding edge has been re-computed and $th^*$ should not exist in $L[u]$. Combining all the costs of all steps, the amortized cost for an update can be deduced as below:
\begin{equation}
\begin{split}
&O(\log n) + O(\log\frac{M+m}{p_f}) + \sum_{w\in N[u]} \frac{O(\log n + \log\frac{M+m}{p_f})}{th} \\
&\leq O(\log n) + O(\log\frac{M+m}{p_f}) + \sum_{w\in N[u]} \frac{O(\log n + \log\frac{M+m}{p_f})}{th^*}\\
  &= O(\log n) + O(\log\frac{M+m}{p_f}) + \frac{d_u}{th^*}O(\log n + \log\frac{M+m}{p_f})\\
  &= O(\log n) + O(\log\frac{M+m}{p_f}) + O(1) \cdot O(\log n + \log\frac{M+m}{p_f})\\
  &= O(\log n + \log\frac{M+m}{p_f})
\end{split}
\end{equation}

\begin{lemma}
\label{lemma:update}
    For any sequence of $M$ updates, the amortized expected update time of our algorithm is bounded by $O(\log n + \log \frac{M+m}{p_f})$.
\end{lemma}

\begin{lemma}
    The index construction takes $O(n + m)$ space. 
\end{lemma}

\noindent\textbf{Linear index space.} We now prove that our algorithm has linear space complexity.
\begin{proof}
    The space required by our index schema consists of $NO$ and $L$. Trivially, the size of $NO$ is bounded by $O(n + m)$. There are $O(n)$ counters for all vertices, and $L[u]$ for each vertex $u$ takes $O(d_u)$ space (each neighbor of $u$ has an element in the bucket). The bucket size is at most $O(d_u)$. The total space cost is then bounded by $O(2n + m + \sum_{u \in V} d_u) = O(2n + m + 2m) = O(n + m)$.
\end{proof}

\noindent\textbf{Remark.} After $M \in O(n^2)$ updates, we can re-set and re-start our algorithm with the updated graph as an input. To start from the sketch, we insert edges (and vertices) from the graph one by one, and each insertion is bounded by $O(\log n + \log\frac{n^2}{p_f}) = O(\log n)$. There are at most $m \in O(n^2)$ insertions that can be charged into the $M$ updates, and the total cost is bounded by $O(\log n)$ amortized expected.

\subsection{$O(n_{cr} + m_{cr})$ query time}\label{subsec:query_time}
To achieve $O(n_{cr} + m_{cr})$ query time, we use the index schema in BOTBIN~\cite{zhang2022effective} that groups the vertices into buckets with $\epsilon$ ranges.
By applying our \emph{RSCM} framework, again $\sigma(u,v)$ is re-computed after $O(d_{max}(u,v))$ updates affecting $(u, v)$, and we only need to update $v$ in at most $\frac{1}{\delta}$ buckets. The  amortized expected time becomes $O(\frac{1}{\delta}\log n + \log \frac{M+m}{p_f})$ = $O(\log n + \log \frac{M+m}{p_f})$, as $\delta$ is a preset constant. We call this method \algoeps.

\begin{lemma}
    The $\epsilon$ bucket index takes $O(n+m)$ space.
\end{lemma}

\begin{proof}
    Each vertex $u$ appears in at most $\frac{1}{\delta}$ buckets. Thus, the total size of the $\epsilon$ bucket index is $\sum_{u \in V}\frac{1}{\delta} = \frac{1}{\delta}n \in O(n+m)$.
\end{proof}

Our \algoeps\ has achieved the best theoretical bounds including linear space complexity, $O(n_{cr} + m_{cr})$ query time, and $O(\log n + \log \frac{M+m}{p_f})$ amortized expected update complexity. However, due to a larger overhead, the update time improvement is less significant compared to \algo. As for \algo, even with an $O(\mu n + m_{cr})$ query time complexity, the practical query time is close to other methods. This is because $n_{cr}$ is close to $n$ in practice, otherwise most vertices are excluded and the clustering results provide limited knowledge to users. We will detail and discuss these in the experiments (Section~\ref{sec:exp}).  

\section{A Lower bound}\label{sec:lb} In this section, we prove that our algorithm matches the worst-case update complexity lower bound of DynStrClu for all parameters. 


\begin{figure}
    \centering
    \begin{subfigure}{0.5\linewidth}
        \includesvg[width=1\textwidth]{figures/new_lower_bound_example1.svg}
        \caption{Before $(v_4, v_7)$ inserted}
        \label{fig:hard_case_exp_a}
    \end{subfigure}%
   \begin{subfigure}{0.475\linewidth}
        
        \includesvg[width=1\textwidth]{figures/new_lower_bound_example2.svg}
        \caption{After $(v_4, v_7)$ inserted}
         \label{fig:hard_case_exp_b}
    \end{subfigure}
    \caption{A hard case example ($\epsilon = 0.5$ and $\mu = 2$)}
    \label{fig:hard_case_exp}
\end{figure}

We first start by constructing a hard instance as shown in Figure~\ref{fig:hard_case_exp}:
\begin{itemize}
    \item $(v_1,v_2) \notin E$;
    \item $|N[v_1]| = \frac{3n}{4}, |N[v_2]| = \frac{3n}{4}$, and all their neighbors are dissimilar to them;
    \item $|N[v_1] \cup N[v_2]| = n$ and $|N[v_1] \cap N[v_2]| = \frac{n}{2}$;
    \item $(v_1, v_2)$ is inserted into the graph as an update.
\end{itemize}

\begin{fact}~\cite{pagh2014min}
\label{fact:lb}
    Given two subsets of $\{1,...,n\}$, the lower bound of one-way communication complexity bits to estimate the Jaccard similarity with a constant probability is $\Omega\left(\frac{n_{max}}{t\Delta^2}\right)$, where $t$ is the intersection size, $n_{max}$ is the size of the larger set, and $\Delta$ is the relative error bound.  
\end{fact}

\begin{lemma}\label{lemma:ins_lb}
    Given two subsets of $\{1,...,n\}$, the lower bound of computation complexity to estimate the Jaccard similarity with a constant probability is $\Omega\left(\frac{n_{max}}{t\Delta^2\log n}\right)$ in the word RAM model.  
\end{lemma}

\begin{proof}
    This can be proved right from Fact~\ref{fact:lb}, as when communicating $\Omega\left(\frac{n_{max}}{t\Delta^2}\right)$ bits, the algorithm must initiate the bits with $\Omega\left(\frac{n_{max}}{t\Delta^2\log n}\right)$ computation complexity.
\end{proof}

\begin{lemma}\label{lemma:no_lazy_update}
    In the worst case, the lower bound cost of estimating the Jaccard similarity with a high success rate can be larger than the cost of outputting the clustering results. 
\end{lemma}

\begin{proof}
     In the hard instance, the similarity calculation of $(v_1, v_2)$ is $\Omega\left(\frac{n}{t\Delta^2\log n}\right)$ with constant probability based on Lemma~\ref{lemma:ins_lb}. To achieve a high success rate ($1-p$), we need to multiply the term by $\log \frac{1}{p}$, making it $\Omega\left(\frac{n_{max}}{t\Delta^2\log n}\log\frac{1}{p}\right)$, where $p$ is a function related to $n$. While the output size is constant ($2$ in Figure~\ref{fig:hard_case_exp_b}).  Hence, Lemma~\ref{lemma:no_lazy_update} holds.
\end{proof}

\begin{lemma}\label{lemma:has_to_comp}
    To achieve a query complexity $O(n_{cr} + m_{cr})$, any correct algorithms need to compute the label of an inserted edge right after it is inserted to guarantee outputting the correct structural clustering results in the worst case.     
\end{lemma}

\begin{proof}
    In the hard instance, once the edge $(v_1, v_2)$ is inserted, the algorithm must know its label, as the label of $(v_1, v_2)$ can immediately change the clustering result,e.g., if it is similar, $v_1$ and $v_2$ are output as a cluster. If a query is right after the update, failing to know the similarity of the inserted edge can lead to a wrong result. With Lemma~\ref{lemma:no_lazy_update}, a lazy update that holds the similarity calculation until computing the output to charge the similarity calculation cost to the output cost is not feasible. Hence, Lemma~\ref{lemma:has_to_comp} holds.
\end{proof}

\begin{lemma} \label{lemma:need_sl}
    To achieve a query complexity $O(n_{cr} + m_{cr})$ for any given $\epsilon$, any correct similarity-computation based algorithms must maintain $NO$ (a linked list to store the neighbors of a vertex sorted by their similarities) for each vertex and support vertex insertion/deletion. 
\end{lemma}

\begin{proof}
    With Lemma~\ref{lemma:has_to_comp}, when $(v_1, v_2)$ is inserted, the algorithm must compute the similarity. Without maintaining sorted relations, $v_2$ is inserted at a random position in $v_1$'s neighbor list. When given an $\epsilon$ for query, the algorithm must scan the whole neighbor list of $v_1$ to decide how many similar neighbors $v_1$ have or it could skip $v_2$ and get the wrong result. Scanning the list takes already $\Omega(n)$. While, based on Section~\ref{subsec:query_time}, with the $NO$, we can achieve a query complexity $O(n_{cr} + m_{cr})$ for any given $\epsilon$. Therefore, Lemma~\ref{lemma:need_sl} holds.
\end{proof}

% \begin{proof}
%     First, the algorithm needs to know all the edge labels, otherwise the output results could be wrong. In the hard instance (Figure~\ref{fig:hard_case_exp_b}), for a $w \in N[v_1]$, if the label of $(v_1, w)$ is similar, it will be included in the cluster, otherwise, it will be excluded out of the cluster. 
    
%     To get all the edge labels when given an $\epsilon$, the algorithm must make an decision on each edge, whether is similarity is below $\epsilon - \rho$ or above $\epsilon + \rho$. Without storing the similarities, the algorithm has to touch each edge and each vertex at least once which takes already $\Omega(n + m)$.  While with the similarities stored, we can apply the algorithm described in Section~\ref{subsec:query_time} to achieve the query complexity $O(n_{cr} + m_{cr})$, hence Lemma~\ref{lemma:need_sc} holds.
% \end{proof}

\begin{lemma}\label{lemma:one_time_es}
    When a graph update occurs, any correct similarity-computation based algorithms must pay at least $\Omega(\log n))$ computation cost in the worst case to maintain a data structure that can output the correct clustering results in $O(n_{cr} + m_{cr})$ time under the $\rho$-approximation with $1-p$ successful rate.
\end{lemma}

\begin{proof}
    This can be derived from Lemma~\ref{lemma:need_sl}, as maintaining the sorted linked list requires $\Omega(\log n)$ in the worst case.
\end{proof}

% \begin{proof}
%     In the hard instance, with Lemma~\ref{lemma:has_to_comp} and Lemma~\ref{lemma:need_sc}, when $(v_1, v_2)$ is inserted, the algorithm must compute the similarity of it, which takes $\Omega\left(\frac{n_{max}}{t\Delta^2}\right)$ based on Lemma~\ref{lemma:ins_lb} with constant probability. Since $\frac{n_{max}}{t} \geq 1$, we can assert the lower bound as $\Omega\left(\frac{1}{\Delta^2}\right)$. In the hard instance, the Jaccard similarity is $\frac{1}{2}$, so we can convert the relative error $\Delta$ into the absolute error $\rho$ by setting $2\rho = \Delta$. Therefore, the lower bound can be represented as $\Omega\left(\frac{1}{4\rho^2}\right) = \Omega\left(\frac{1}{\rho^2}\right)$, or $\Omega\left(\frac{1}{\rho^2}\log\frac{1}{p}\right)$ to ensure a high success rate. Hence Lemma~\ref{lemma:one_time_es} holds.
% \end{proof}

\begin{lemma}
    Our \algo matches the update complexity lower bound of the dynamical structural clustering for all parameters problem when $p_f = \frac{1}{n})$. 
\end{lemma}

\begin{proof}
    As described in Section~\ref{subsec:for_all_p}, our algorithm achieves an amortized $O\left(\log n + \log \frac{M+m}{p_f}\right)$ update complexity which matches the lower bound $\Omega(\log n)$ when $p_f = \frac{1}{n}$. This is because when $M$ is smaller than $n$, $\log \frac{M+m}{p_f} \in O(\log n)$, while when $M$ is greater than $n$, we can re-set and re-start our algorithm to achieve $O(\log n)$ amortized complexity based on Section~\ref{subsec:for_all_p}.
\end{proof}


% \begin{proof}
%      With Lemma~\ref{lemma:one_time_es}, the lower bound complexity to a data structure that can output the correct clustering results in $O(n_{cr} + m_{cr})$ time under the $\rho$-approximation with $1-p_f$ successful rate for $M$ times estimation is $\Omega\left(\frac{1}{\rho^2}\log\frac{M}{p_f}\right)$ based on the Union Bound by setting $p = \frac{p_f}{i(i+1)}$ where $i$ is the $i^{th}$ estimation. As described in Section~\ref{subsec:for_all_p}, our algorithm achieves an amortized $O\left(\log n + \log \frac{M}{p_f}\right)$ update complexity which matches the lower bound when $p_f = \frac{1}{n})$. This is because when $M$ is smaller than $n$, $\log \frac{M}{p_f} \in \Theta(\log n)$, while when $M$ is greater than $n$, $\log n \in O\left(\log \frac{M}{p_f}\right)$.
% \end{proof}




\section{Accommodating Cosine Similarity}
\label{subsec:cos}
We now extend our algorithms to using cosine similarity as the similarity measure. DICE similarity is an easier case and the analysis is put in the technical report due to space limit.

We first modify the sampling method in similarity estimation to satisfy the $O(\log \frac{M}{p_f})$ time complexity, then deduce the number of impacting updates for an edge under the cosine similarity setting, and lastly discuss how to fit cosine similarity in on-the-fly parameter schema.    

\subsection{Similarity Estimation}
We first propose a sampling-based method for estimating the cosine similarity.

Consider an arbitrary edge $(u,v)$; let $a = |N[u]\cap N[v]|$, $b_1 = |N[u]|$, and $b_2 = |N[v]|$. Without losing the generality, we assume $b_2$ is not smaller than $b_1$. We define a random variable $X$ which is generated by the following steps:
\begin{enumerate}
    \item Draw a vertex $w$ from $N[v]$ uniformly at random.  
    \item Check if $w \in N[u]$, if so, $X=1$m; otherwise $X=0$.
\end{enumerate}
From the procedures, we have $Pr[X=1] = \frac{a}{b_2}$.
Let $X_1, X_2, ... X_L  $ be $L$ independent instances of the random variable $X$, and define $\Bar{X} = \frac{1}{L}\sum_{i=1}^LX_i$. We have:
$$E[\Bar{X}] = \frac{a}{b_2} = \frac{\sqrt{\frac{b_1}{b_2}}a}{\sqrt{b_1b_2}}\rightarrow\sigma_c(u,v) = \sqrt{\frac{b_2}{b_1}}E[\Bar{X}]$$

We now prove that, with this sampling method, we can estimate the similarity in $O(\log\frac{2}{p})$ time. We consider the estimation in two cases:

(1) When $\min(d_u,d_v) < \epsilon^2\max(d_u,d_v)$, we can instantly label $u$ and $v$ as dissimilar, as $\sigma_c(u,v) = \frac{|N[u]\cap N[u]|}{\sqrt{d_u\cdot d_v}} < \frac{\min(d_u, d_v)}{\sqrt{d_u\cdot d_v}} <  \frac{\min(d_u, d_v)}{\sqrt{\frac{1}{\epsilon^2}\min(d_u, d_v)^2}} = \epsilon$. 

(2) When $\min(d_u,d_v) \geq \epsilon^2\max(d_u,d_v)$, we would like to compute the probability when the estimated similarity is out of the error bound, that is: 
$$Pr[|\Tilde{\sigma}(u,v) -\sigma(u,v)| > \rho]$$
Substitute with $\Bar{X}$, and we have:
$$Pr[\sqrt{\frac{b_2}{b_1}}|\Bar{X} - E[\Bar{X}]| > \rho]$$
As $\min(d_u,d_v) \geq \epsilon^2\max(d_u,d_v) \rightarrow \sqrt{\frac{b_2}{b_1}} \leq \frac{1}{\epsilon}$, we can get:
$$Pr[\sqrt{\frac{b_2}{b_1}}|\Bar{X} - E[\Bar{X}]| > \rho] \leq Pr[|\Bar{X} - E[\Bar{X}]| > \rho\epsilon]=p$$ 
By Hoeffding bound~\cite{hoeffding1994probability}, when the sample size $k = \frac{2}{\epsilon^2\rho^2}\ln{\frac{2}{p}}$, we have $Pr[|\Tilde{\sigma(u,v)} - \sigma(u,v)| > \rho] ]\leq p$. 

However, the deduced $k$ is related to $\epsilon$ which is an input parameter. To remove $\epsilon$ dependency from $k$, we discuss two cases:

(1) When $\epsilon \leq \rho$, we instantly get the clustering result as all edges can be labeled as similar due to $\sigma(u,v) > \epsilon - \rho $. 

(2) When $\epsilon > \rho$, it is safe to select $k = \frac{2}{\rho^4}\ln{\frac{2}{p}}$ which is not smaller than $\frac{2}{\epsilon^2\rho^2}\ln{\frac{2}{p}}$. 

As we need to sample twice in each neighbor, the time complexity is $O(2k) = \frac{4}{\rho^4}\ln{\frac{2}{p}} \in O(\log\frac{2}{p})$ that is the same as Jaccard Similarity.
% \begin{fact}[\cite{ruan2021dynamic}]
% \label{fact:sim}
%     Let $X_1, X_2, ... X_L  $ be $L$ independent instances of the random variable $X$, and define $\Bar{X} = \frac{1}{L}\sum_{i=1}^LX_i$. There exists a sampling method that has:
%     $$\frac{|N[u]\cap N[u]|}{|N[u]\cup N[u]|} = \frac{E[\Bar{X}]}{2-E[\Bar{X}]}$$
% \end{fact}

% By Fact~\ref{fact:sim}, we can use the same sampling method in~\cite{ruan2021dynamic} for the cosine similarity estimation but calculate it as $\hat{\sigma}_c(u,v) = \frac{(d_u + d_v)\Bar{X}}{2\sqrt{d_u\cdot d_v}}$. This can be deduced from:

% $$|N[u]\cap N[u]| = d_u + d_v - |N[u]\cup N[u]| = \frac{1}{2}(d_u + d_v)E[\Bar{X}]$$
% And we have:

% $$\sigma_c(u,v) = \frac{|N[u]\cap N[u]|}{\sqrt{d_u\cdot d_v}} = \frac{(d_u + d_v)E[\Bar{X}]}{2\sqrt{d_u\cdot d_v}}$$

% We now prove that, with this sampling method, we can still estimate the similarity in $O(\log\frac{2}{p})$ time. We consider the estimation in two cases:

% (1) When $\min(d_u,d_v) < \epsilon^2\max(d_u,d_v)$. In this case, we can instantly label $u$ and $v$ as dissimilar, as $\sigma_c(u,v) = \frac{|N[u]\cap N[u]|}{\sqrt{d_u\cdot d_v}} < \frac{\min(d_u, d_v)}{\sqrt{d_u\cdot d_v}} <  \frac{\min(d_u, d_v)}{\sqrt{\frac{1}{\epsilon^2}\min(d_u, d_v)^2}} = \epsilon$. 

% (2) When $\min(d_u,d_v) \geq \epsilon^2\max(d_u,d_v)$. In this case, we would like to compute the probability when the estimated similarity is out of the error bound, that is: 
% $$Pr[|\Tilde{\sigma}(u,v) -\sigma(u,v)| > \rho]$$
% Substitute with $\Bar{X}$, and we have:
% $$Pr[\frac{d_u + d_v}{2\sqrt{d_u \cdot d_v}}|\Bar{X} - E[\Bar{X}]| > \rho]$$
% As $\frac{d_u + d_v}{\sqrt{d_u \cdot d_v}} \leq \epsilon + \frac{1}{\epsilon}$, we can get:
% $$Pr[\frac{d_u + d_v}{2\sqrt{d_u \cdot d_v}}|\Bar{X} - E[\Bar{X}]| > \rho] \leq Pr[|\Bar{X} - E[\Bar{X}]| > \frac{2\rho}{\epsilon + \frac{1}{\epsilon}}]=p$$ 
% By Hoeffding bound~\cite{hoeffding1994probability}, when the sample size $k = \frac{(\epsilon + \frac{1}{\epsilon})^2}{8\rho^2}\ln{\frac{2}{p}}$, we have $Pr[|\Tilde{\sigma(u,v)} - \sigma(u,v)| > \rho] ]\leq p$. 

% However, the deduced $k$ is related to $\epsilon$ which is an input parameter. To remove $\epsilon$ dependency from $k$, we discuss two cases:

% (1) When $\epsilon \leq \rho$, we instantly get the clustering result as all edges can be labeled as similar due to $\sigma(u,v) > \epsilon - \rho $. 

% (2) When $\epsilon > \rho$, it is safe to select $k = \frac{(\rho + \frac{1}{\rho})^2}{8\rho^2}\ln{\frac{2}{p_f}}$ which is not smaller than $\frac{(\epsilon + \frac{1}{\epsilon})^2}{8\rho^2}\ln{\frac{2}{p_f}}$. This can be easily proven by the monotonicity of the function $f(x) = x + \frac{1}{x}$ in the range $(0, 1)$.
% % \begin{itemize}
% %     \item set $y = x + \frac{1}{x}$
% %     \item $y' = 1 - \frac{1}{x^2}$
% %     \item $\epsilon$ and $\rho$ are both in $(0,1)$
% %     \item when $0 \leq x \leq  1$, $y' \leq 0$
% %     \item the value of $y$ decrease when $x$ increase in this range
% %     \item when $\epsilon > \rho$, $\epsilon + \frac{1}{\epsilon} < \rho + \frac{1}{\rho}$
% % \end{itemize}

% As we need to sample twice in each neighbor, the time complexity is $O(2k) = \frac{(\rho + \frac{1}{\rho})^2}{4\rho^2}\ln{\frac{2}{p}} \in O(\log\frac{2}{p})$ that is the same as Jaccard Similarity.

%We propose a sampling method using cosine similarity.
% When estimating the similarity between  vertex $u$ and vertex $v$, we let $a = |N[u]\cap N[v]|$, $b_1 = |N[u]|$, and $b_2 = |N[v]|$, and the sampling steps run as follows. 
% \begin{itemize}
%     \item We uniformly randomly pick a vertex from $N[u]$, denoted as $w_1$;
%     \item If $w_1 \in N[u] \cap N[v]$, then $z_1 = 1$; otherwise, $X_1 = 0$;
%     \item We uniformly randomly pick a vertex from $N[v]$, denoted as $w_2$;
%     \item If $w_2 \in N[u] \cap N[v]$, then $z_2 = 1$; otherwise, $X_2 = 0$;
%     \item Let $X=1$ only when $z_1 = 1 \wedge z_2 = 1$.
% \end{itemize}
% Based on the steps, 
% \begin{align}
%     Pr[X=1] &= Pr[z_1 = 1 \wedge z_2 = 1]\\
%             &= \frac{a}{b_1} \cdot \frac{a}{b_2} = \frac{a^2}{b_1b_2}
% \end{align}
% Denote $X_k$ as the $k^{th}$ independent instance of $X$, and we have $\Bar{X} = \frac{1}{k}\Sigma^k_{i=1}X_i$, and $E[\Bar{X}] = \sigma(u,v)^2.$

% $X_i$ is independent and $\Bar{X}$/$E[\Bar{X}]$ are bounded by $[0, 1]$, based on Hoeffding Bound~\cite{hoeffding1994probability}, $Pr[|\Bar{X} - E[\Bar{X}]| > \triangle] \leq p$ when $k = \frac{1}{2\triangle^2}\ln\frac{2}{p}$. Here, $\Bar{X} = \Tilde{\sigma}(u, v)^2$, and we have when:

% $$|\sigma(u, v)^2 - \Tilde{\sigma}(u, v)^2| \leq \triangle$$ 
% $$(\sigma(u, v) - \Tilde{\sigma}(u, v))^2 = \sigma(u, v)^2 - \Tilde{\sigma}(u, v)^2 - 2\sigma(u, v)\Tilde{\sigma}(u, v) + 2\Tilde{\sigma}(u, v)^2$$ $$\rightarrow 0 \leq (\sigma(u, v) - \Tilde{\sigma}(u, v))^2 < \triangle + 2$$ $$\rightarrow |\sigma(u, v) - \Tilde{\sigma}(u, v)| < \sqrt{\triangle + 2}$$
% If we set $\triangle = \rho^2 - 2$, we will have $Pr[|\sigma(u,v) - \Tilde{\sigma}(u,v)]| > \rho] \leq p_f$, and $k = \frac{1}{2(\rho^2 - 2)^2}\ln\frac{2}{p}$. 




\subsection{Update Affordability}
We now analyze the update affordability under cosine similarity. 

When edge $(u,w)$ is inserted, let $(u,v)$ be an arbitrary edge affected by the update, where $v \in N[u]$. Let $a = |N[u]\cap N[v]|$, $b_1 = |N[u]|$, and $b_2 = |N[v]|$. The possible changes of $\sigma(u, v)$ are:
    \begin{enumerate}
        \item $\frac{a+1}{\sqrt{(b_1 + 1)b_2}}$ or $\frac{a+1}{\sqrt{b_1(b_2 + 1)}}$
        \item $\frac{a}{\sqrt{(b_1 + 1)b_2}}$ or $\frac{a}{\sqrt{b_1(b_2 + 1)}}$
    \end{enumerate}
As for deletion, it could be:
    \begin{enumerate}
        \item $\frac{a-1}{\sqrt{(b_1 - 1)b_2}}$ or $\frac{a-1}{\sqrt{b_1(b_2 - 1)}}$
        \item $\frac{a}{\sqrt{(b_1 - 1)b_2}}$or $\frac{a}{\sqrt{b_1(b_2 - 1)}}$
    \end{enumerate}
Among these changes, it is trivial to prove that case (1) in insertion and case (2) in deletion are increments, while case (2) in insertion and case (1) in deletion are reductions. Without loss of generality, we assume that $b_2$ is not smaller than $b_1$. To prove that $\frac{a+1}{\sqrt{(b_1 + 1)b_2}}$ has the maximum increment, we have:

 % $$\frac{a+1}{\sqrt{(b_1 + 1)b_2}} > \frac{a}{\sqrt{(b_1 + 1)b_2}}$$
 % $$\frac{a-1}{\sqrt{(b_1 - 1)b_2}} < \frac{a}{\sqrt{(b_1 - 1)b_2}}$$
 
\begin{equation} \label{eq2}
\begin{split}
&\frac{\frac{a+1}{\sqrt{(b_1 + 1)b_2}}}{\frac{a}{\sqrt{(b_1 - 1)b_2}}}
 =\frac{a+1}{a}\sqrt{\frac{b_1 -1}{b_1 + 1}}
 =  \frac{a+1}{a}\sqrt{\frac{(b_1 -1)^2}{b_1^2 - 1}} \\
 = &\frac{a+1}{a}\frac{b_1 -1}{\sqrt{b_1^2 - 1}}
 > \frac{a+1}{a}\frac{b_1 -1}{\sqrt{b_1^2}} = \frac{a+1}{a}\frac{b_1 -1}{b_1}\\
 = &1 + \frac{b_1 -a - 1}{ab_1}
\end{split}
\end{equation}

Note that $u$ has at least one neighbor which is not shared with $v$ to make the $\frac{a}{\sqrt{(b_1 - 1)b_2}}$ possible, so we have $b_1 \geq a + 1$ and $1 + \frac{b_1 -a - 1}{ab_1} \geq 1$, hence
$\frac{a+1}{\sqrt{(b_1 + 1)b_2}} > \frac{a}{\sqrt{(b_1 - 1)b_2}}$. Otherwise, if $b_1 = a$, $\frac{a+1}{\sqrt{(b_1 + 1)b_2}}$ is the only case that increases $\sigma(u,v)$. Therefore, we have $\frac{a+1}{\sqrt{(b_1 + 1)b_2}}$ gets the most increase for one update.

After $M$ updates, in the worst case, $\sigma(u,v)$ can be increased to $\frac{a+M}{\sqrt{(b_1 + M_1)(b_2+M_2)}}$ where $M_1 + M_2 = M$. We select $k$ to satisfy $\frac{1}{2}\rho$-approximation in our estimation algorithm, and we need to find out the maximum $M$ that will not change the clustering results for any given $\epsilon$.
That is:
$$\max_M\{\frac{a+M}{\sqrt{(b_1 + M_1)(b_2+M_2)}}\} \leq \epsilon + \rho$$

As we mentioned in the last section, when $b_1 < \epsilon^2b_2$, we can instantly label $u$ and $v$ as dissimilar. Hence, we only discuss the case when $b_1 \geq \epsilon^2b_2$. With $b_1 \geq \epsilon^2 b_2\rightarrow \sqrt{b_1b_2} \geq \sqrt{\epsilon^2b_2^2} = \epsilon b_2$, we have $\frac{M}{\sqrt{b_1b_2}} \leq \frac{M}{\epsilon b_2}$. If we set $M \leq \frac{1}{2}\rho\epsilon b_2$, then $\frac{M}{\sqrt{b_1b_2}} < \frac{1}{2}\rho$. Hence, when $M \leq \frac{1}{2}\rho\epsilon b_2$, we have:

\begin{small}
\begin{equation} \label{eq}
\begin{split}
\frac{a+M}{\sqrt{(b_1 + M_1)(b_2+M_2)}} &= \frac{a}{\sqrt{(b_1 + M_1)(b_2+M_2)}} + \frac{M}{\sqrt{(b_1 + M_1)(b_2+M_2)}}\\
& <  \frac{a}{\sqrt{b_1 b_2}} + \frac{M}{\sqrt{b_1b_2}}\\
& < \epsilon + \frac{1}{2}\rho + \frac{1}{2}\rho
\end{split}
\end{equation}
\end{small}

To conclude, after $\lfloor \frac{1}{2}\epsilon\rho\cdot\max(d_u, d_v)\rfloor$ affecting updates, the maximum similarity increment will not exceed $\frac{1}{2}\rho$ with a probability $1-p$. A similar proof can be done for maximum decrement, which is omitted. 

To support on-the-fly parameters, $\epsilon$ becomes an input parameter and cannot be considered a constant. As we mentioned above, when $\epsilon < \rho$, we can label all edges as similar edges. While when $\epsilon \geq \rho$, $ \frac{1}{2}\epsilon\rho \cdot max(d_u, d_v) \geq \frac{1}{2}\rho^2 \cdot max(d_u, d_v)$. It is safe to set  $th(u, v) = 2^{\lfloor\log_2{\frac{1}{4}\rho^2 \cdot \max(d_u,d_v)\rfloor}} \in O(\max(d_u, d_v))$, so that edge $(u, v)$ will be re-computed before changing its similar edge status for any given $\epsilon$ under our \emph{RSCM} framework. 

\begin{lemma}
\label{lemma:cos}
     When measuring cosine similarity, with probability $\geq 1 - p$, an edge $(u, v)$ can afford at least $\ell = \lfloor \frac{1}{2}\rho^2\cdot\max(d_u, d_v)\rfloor$ affecting updates before it changes from a similar edge to a dissimilar one, and vice versa for any given $\epsilon$.    
\end{lemma}

\section{Optimizations}
\label{sec:opt}
We further describe three optimization methods that can improve the practical running time.

\subsection{Group Vertex by Degree}
For our \algo, we need to scan all vertices to decide whether they are core vertices. A simple and effective way to accelerate the computation is to maintain a bucket structure that groups the vertices by their degrees, i.e., with buckets for degree ranges of $[2, \Bar{d}], (\Bar{d}, 2\Bar{d}], \ldots$, where $\Bar{d}$ is the average degree of the dataset. Each vertex is put into a corresponding bucket based on their degree. In this way, given $\mu$, we can quickly locate the bucket to which $\mu$ belongs. All the buckets before it can be skipped as the vertices in them cannot be core vertices satisfying $\mu$. Maintaining this bucket takes an extra $O(m)$ space, and our method is still linear to the graph size in terms of space cost, while an update operation takes $O(1)$ time to maintain the buckets. 


\subsection{Small $\mu$ Table}
\label{subsubsec:opt_3}
In many applications, $\mu$ is usually chosen as a small value comparing to $n$ and $m$, e.g., $\mu=5$ while $n$ and $m$ are greater than a million as in previous studies~\cite{xu2007scan,ruan2021dynamic, wen2017efficient, zhang2022effective}. For the $\mu$ table index~\cite{wen2017efficient}, we do not need to store all the possible $\mu$ rows each of which takes $O(d)$ space in the worst case. We can maintain a constant size $\mu$ table that covers most query cases, hence achieving an $O(n_{cr} + m_{cr})$ query time complexity for those queries. When the queried $\mu$ is larger than what we keep, we can use our \algo~to get the result in $O(\mu n + m_{cr})$ time. In this way, the amortized update time complexity is still $O(\log n + \log \frac{M+m}{p_f})$ applying our \emph{RSCM} with constant size $\mu$ table.

To further analyze the update complexity, we formulate the probability of $\mu$ as $p_{\mu}= \frac{1}{\mu\ln n}$ with $2 \leq \mu \leq n$, hence $\sum_{\mu=2}^np_u <\int_1^np_{\mu}d\mu = 1$. The larger the $\mu$ is, the smaller the probability. 

If the $\mu$ table size is set to $\mu'$, the expected query cost can then be represented as:
\begin{small}
\begin{equation}
    \begin{split}
        m_{cr} + \sum_{\mu = 2}^{\mu'}p_\mu n_{cr} + \sum_{\mu = \mu'}^{n}p_\mu \mu n
        &= m_{cr} + \sum_{\mu = 2}^{\mu'}\frac{1}{\mu \ln n} n_{cr} + \sum_{\mu = \mu'}^{n}\frac{1}{\mu \ln n} \mu n\\
        &< m_{cr} + \int_{2}^{\mu'}\frac{1}{\mu \ln n} n_{cr} d\mu + \sum_{\mu = \mu'}^{n}\frac{1}{\mu \ln n} \mu n\\
        &< m_{cr} + \frac{\ln \mu'}{\ln n}n_{cr} + \frac{n(n-\mu')}{\ln n}\\
    \end{split}
\end{equation}   
\end{small}


We call this method \algomu.

\subsection{Ratio of $\rho$ Allocation}
\label{subsubsec:opt_1}
First, we consider only our \algo. There are two parts of approximation in our algorithms:
\begin{itemize}
    \item In similarity estimation, the sample size $k$ is selected as $\frac{2}{\rho_1^2}\ln{\frac{2}{p}}$ to bound the absolute error less than $\rho_1$.
    \item In \emph{RSCM}, $th$ is set to $2^{\lfloor\log_2{\frac{1}{4}\rho_2\max(d_u,d_v)\rfloor}}$ to assure that $\sigma(u, v)$ is changed by less than $\rho_2$ before re-computation.
\end{itemize}

We set $\rho_1 + \rho_2 = \rho$ to satisfy $\rho$-approximation for our algorithm. As $\rho$ is a constant, the ratio of $\rho_1$ to $\rho_2$ does not impact the theoretical time complexity. However, there exists a ratio to minimize the constant factor of the complexity. Refer to Lemma~\ref{lemma:update}, the amortized update time is $O(\log n) +   \frac{2}{\rho_1^2}\log \frac{M+m}{p_f} + (\frac{2}{\rho_2} + 1)(\log n + \frac{2}{\rho_1^2}\log \frac{M+m}{p_f})$. We consider that $\log n$ and $\log \frac{M+m}{p_f}$ are of the same magnitude, and our goal is to select $\rho_1$ and $\rho_2$ to minimize $\frac{2}{\rho_2} + \frac{4}{\rho_1^2\rho_2} + \frac{4}{\rho_1^2}$ with $\rho_1 + \rho_2 = \rho$ and $0 < \rho < 1$. When $\rho$ is given, we can quickly calculate $\rho_1$ and $\rho_2$. For example, when $\rho = 0.02$ we have $\rho_1 = 0.0134$ and $\rho_2 = 0.0066$.

Now we consider \algoeps. As described before, the $\epsilon$-bucketing introduces a $\delta$ absolute error in similarity estimation, hence we need to set $\rho_1 + \rho_2 + \delta = \rho$, and our goal is to minimize $\frac{2}{\delta\rho_2} + \frac{4}{\delta\rho_1^2\rho_2} + \frac{2(1+\frac{1}{\delta})}{\rho_1^2}$. When $\delta$ is given, the calculation is similar to the above but with different constant factors. 
%For example, if $\rho=0.02, \delta = 0.01$, we can have $\rho_1 = 0.0133$ and $\rho_ = 0.0067$.

% \subsection{Discussion}
% For our \algo~and its variants, handling vertex insertion is straightforward. Additionally, we do not assume the graph update pattern for our complexity claim.

% \noindent\underline{New vertex insertion.} For our algorithm, inserting a new vertex $u$ has no difference from inserting an edge between existing vertices except that $NO[u]$ with only $u$ in it and an empty $L[u]$ are created before conducting our algorithm, which takes $O(1)$. 

% \noindent\underline{Update pattern.} Our algorithm can keep the amortized update cost under any update pattern. Even with repeatedly the same edge updates, e.g., repeatedly removing and inserting the same edge $(u,v)$, the update amortized cost still holds as the similarity between $u$ and its neighbor are re-computed only after enough amount affected updates under our \emph{RSCM} framework. 



==> sections/backup-SOTA_algorithms.tex <==
\subsection{A Unified Algorithm Framework}

For ease of presentation, we 
introduce 
a {\em unified algorithm framework} for solving {\em DynStrClu-AllPara}, 
whose pseudo-code is shown in Algorithm~\ref{algo:framework}.
Both the state-of-the-art exact and approximate algorithms discussed in this paper, as well as our proposed solutions,
%in subsequent sections, 
all work under this framework.
%present the state-of-the-art exact and approximate algorithms for {\em DynStrClu-AllPara} under a {\em unified algorithm framework} whose pusedo-code is shown in Algorithm~\ref{algo:framework}.
%As we shall see in Section~\ref{sec:our-algo}, our proposed algorithm also follows this algorithm framework.
%
At high level, these algorithms implement the following data structures:
%which consists of two main components: 
\begin{itemize}[leftmargin = *]
\item {\bf \em Sorted Neighbor Lists}: for each vertex $u \in V$, a {\em non-increasing sorted} list of $u$'s neighbors by their similarities to $u$; with a slight abuse of notation, we simply use $N(u)$ to refer to this sorted list, and each neighbor $v$ of $u$ in this list is stored along with its similarity to $u$. 
%\item an edge similarity maintenance structure which:
%\begin{itemize}
\item {\bf \em EdgeFindStr}: a data structure for maintaining the (approximate) similarities for all the edges;
there are three functions:
\begin{itemize}
\item update($(u,v)$, $op$): given an update of edge $(u,v)$, where $op$ indicates whether this is an insertion or deletion, update~{\em EdgeFindStr};
\item find($(u,v)$, $op$): return the set $F$ of all the affected edges whose similarities are needed to be re-computed;
\item cal-sim($(x, y)$): given an edge $(x, y)$, return $\sigma(x,y)$;  
\end{itemize} 
%\item keeps a {\em sorted} neighbor  list, for each vertex $u$, in a {\em non-increasing} order by their similarities to $u$. 
%\end{itemize}
\item {\bf \em CoreFindStr}: a data structure for finding core vertices; there are two functions:
\begin{itemize}
\item update($u$): given a vertex $u \in V$, update {\em CoreFindStr} for $u$;
\item find-core($\eps$, $\mu$): return the set $\Vc$ of all the core vertices with respect to the given parameters $\eps$ and $\mu$; 
\end{itemize}
\end{itemize}
%These modules aim to support 
%The goal of maintaining these data structures is to answer each query with parameters $\eps$ and $\mu$ by outputting the corresponding clustering result in $O(|E_{cr}|)$ time.
%
%All the algorithms discussed in this paper differ only the implementations of {\em EdgeSimStr} and {\em CoreFindStr}, and hence, achieve different running time bounds on handling each update and query.


\input{sections/algo-framework}


\vspace{1mm}
\noindent
{\bf Running Time Analysis.}
Let
$\costeu$, $\costef$ and $\costec$ denote the running time cost of each invocation of the functions {\em update}, {\em find} and {\em cal-sim} in {\em EdgeSimStr}, repectively;
and $\costcf$ and $\costcu$ denote the running time cost of each invocation of the functions {\em find-core}
and {\em update} in {\em CoreFindStr}, respectively.

\vspace{1mm}
\noindent
\underline{\em Query Running Time.}
Clearly, by Observation~\ref{fact:clustering-graph}, the running time cost for each query is bounded by 
$O(\costcf + m_{cr})$.

\vspace{1mm}
\noindent
\underline{\em Per-Update Running Time.}
In the Update Procedure in Algorithm Framework~\ref{algo:framework},
Line~2 takes $O(\costeu)$ time and Lines~3-7 takes $O(\costec + \log n)$ time, where $O(\log n)$ is the maintenance cost for the sorted neighbor lists.
Furthermore, the running time cost of Line~8 
is bounded $O(\costef)$ while that of Lines 9-11  is bounded by $O(|F| \cdot (\costec + \log n))$. 
Finally, Lines 13 - 14 can be performed in $O(|F| \cdot \costcu)$ because $|S| \in O(|F|)$. 
Summing all these costs up, 
the overall running time of each update is bounded by 
\begin{equation}\label{eq:query-bound}
O\left(\costeu + (|F| + 1) \cdot (\costec + \log n + \costcu)\right)\,.
\end{equation}

In the following, we just need to focus on the implementations of {\em EdgeSimStr} and {\em CoreFindStr} of different algorithms.
And putting their corresponding operation costs in the above analysis, the query and per-update running time bound follow.
 

\begin{comment}
\vspace{1mm}
\noindent
{\bf Answering Queries.}
Specifically, for any given query parameters $\eps$ and $\mu$, 
the Query Procedure in the unified algorithm framework Algorithm~\ref{algo:framework} works as follows.
Firstly, retrieve the set $\Vc$ of all the core vertices with {\em CoreFindStr}. 
Secondly, for each vertex $u \in \Vc$, scan the sorted neighbor list of $u$ and add all the sim-edge of $u$ to $E_{cr}$.
Finally, compute and return the clustering result from the induced graph $G_{cr}$ by $E_{cr}$ according to Observation~\ref{fact:clustering-graph}.
\end{comment}

\begin{comment}
\vspace{1mm}
\noindent
\underline{\em Query Time Analysis}. 
Denote the running time cost for finding $\Vc$ in the first step of the Query Procedure by $Cost_{\text{CoreFind}}$.
Clearly, the second and third steps can be performed in $O(|E_{cr}|)$ time.
Therefore, overall running time for answering each query is bounded by $O(Cost_{\text{CoreFind}} + |E_{cr}|)$.  
\end{comment}

\begin{comment}
\vspace{1mm}
\noindent
{\bf Handling Updates.}
For an update of edge $(u,v)$, 
the Update Procedure performs the following steps:
\begin{itemize}[leftmargin = *]
\item {\bf Step 1.1:} if this update is an insertion, then: 
\begin{itemize}
\item compute $\sigma(u,v)$, 
\item add $(u,v)$ to $E$, and 
\item insert $v$ to the sorted neighbor list of $u$ (and $u$ to $v$'s sorted neighbor list, respectively);
\end{itemize}
\item {\bf Step 1.2:} if this update is a deletion, then (i) remove edge $(u,v)$ from $E$ and (ii) remove $v$ (resp., $u$) from the sorted list neighbor list of $u$ (resp., $v$);
\item {\bf Step 2:} identify the set, denoted by $F$, of all the affected edge whose similarities become ``invalid'' due to the update of $(u,v)$ and need to be re-calculated;
\item {\bf Step 3:} re-calculate the similarity of each edge in $F$ and update the sorted neighbor lists accordingly;
%\item {\bf Step 3.2:} 
%whose similarity becomes ``invalid'';
\item {\bf Step 4:} update {\em CoreFindStr} for all those end-vertices of the edges in $F$ plus $u$ and $v$;
% which have similarities to some neighbors re-computed; 
\end{itemize}
%
The only differences among the state-of-the-art algorithms and our proposed solutions
are in the implementations of 
%\begin{itemize}[leftmargin = *]
(i) ``invalid'' affected edge identification (Step 2), 
(ii) edge similarity calculation (Step 3), 
and (iii) {\em CoreFindStr} for $\Vc$ retrieval and the structure update (Step 4).
%which includes the implementations of the update (Step 4) and $\Vc$ retrieval. 
%\end{itemize}
\end{comment}

\subsection{A State-of-the-Art Exact Algorithm}
\label{sec:gsindex}

%\input{figures/figure_scripts/indexing_example}

The {\em GS*-Index}~\cite{wen2017efficient} 
is a state-of-the-art exact algorithm for the {\em DynStrClu-AllPara} problem. 
Its implementations
of {\em EdgeSimStr} and {\em CoreFindStr} are as follows.





\vspace{1mm}
\noindent
{\bf The Implementation of {\em EdgeSimStr}.}
For each vertex $u \in V$, the {\em EdgeSimStr} in GS*-index maintains $d_u$, the degree of $u$, and $I(u,x)$, the {\em intersection size} of $N[u]$ and $N[x]$, for each neighbor $x \in N(u)$. 
%Clearly, the simialrity $\sigma(u,v)$ can be computed with $I(u,v)$, $d_u$ and $d_v$ in $O(1)$ time.
And the three functions 
are implemented as follows:
\begin{itemize}[leftmargin = *]
\item update($(u,v)$, $op$): maintain the counters $d_u$ and $I(u,x)$ for each $x \in N(u)$ according to the given update. Perform the same maintenance symmetrically for the end-vertex $v$.
Therefore, $\costeu \in O(d_u + d_v) \subseteq O(d_{\max})$, where $d_{\max}$ is the largest degree of $G$.

\item find($(u,v)$, $op$): 
return the set of all the affected edges of the update $(u,v)$.
Hence, $|F| \in O(d_u + d_v)$ and hence, $\costef \in O(d_{\max})$.

\item cal-sim($(x, y)$): as discussed earlier, $\sigma(u,v)$ can be computed with $I(u,v)$, $d_u$ and $d_v$.
Thus, $\costec \in O(1)$. 
\end{itemize}

\vspace{1mm}
\noindent
{\bf The Implementation of {\em CoreFindStr}}: The GS*-index implements the {\em CoreFindStr} as a {\em $\mu$-Table}, denoted by $T$, which is essentially an array of $d_\max$ sorted lists.
Specifially, for integer $1 \leq i \leq d_\max$, $T[i]$ stores a {\em sorted} list of all the vertices $u$ (with degrees $d_u \geq i$) in a {\em non-increasing} order by 
%$\eps_{u, i}$, 
%where $\eps_{u,i}$ is   
the $i^\text{th}$ largest similarity of $u$ to its neighbors, denoted by $\eps_{u,i}$.
%by the similarity values $\eps_{u, i}$.
%the $i^\text{th}$ {\em largest} similarity to their neighbors. 
\begin{itemize}[leftmargin = *]
\item find-core($\eps$, $\mu$): 
%The rationale of the $\mu$-Table is that, 
%given parameters $\eps$ and $\mu$,
retrieve all the core vertices 
by scanning and reporting the vertices in the sorted list $T[\mu]$ until the first vertex $x$ such that $\eps_{x, \mu} < \eps$ is met or the entire list has been retrieved.
As a result, $\costcf \in O(|\Vc| + 1)$.

\item update($x$): maintain the sorted lists $T[1], \cdots, T[d_x]$ for $x$ accordingly. This takes $\costcu \in O(d_{\max}\cdot \log n)$ time, because the maintenance on each of these sorted lists takes $O(\log n)$ time. 
\end{itemize}
%
Substituting the running time costs of the above implementations, 
it can be verified that:
\begin{fact}
The GS*-index can answer each query in $O(m_{cr})$ time and can handle each update in $O(d^2_{\max} \cdot \log n)$ time with space consumption bounded by $O(n + m)$ at all times.
\end{fact}

\subsection{A State-of-the-Art  Approximate Algorithm}
\label{sec:botbin}

%While the space consumption and the query time complexity of GS*-index are good,
Unfortunately, the $O(d_{\max}^2 \cdot \log n)$ per-update time of GS*-index is prohibitive as $d_{\max}$ can be as large as $n$.
To remedy this, BOTBIN~\cite{} adopts a notion of {\em $\rho$-absolute-approximation}
%which is extended from the $\rho$-relative-approximation proposed in~\cite{} 
for the {\em DynStrClu-AllPara} problem, and dramatically improved the per-update cost from $O(d_{\max}^2 \cdot \log n)$ to roughly $O(\log^2 n)$ {\em in expectation}.
However, BOTBIN only works for Jaccard similarity measurement and this expected update bound only holds under an assumption that the updates on $G$ are {\em uniform at random}.

\vspace{1mm}
\noindent{\bf $\rho$-Absolute-Approximation.}
%The overcome these challenges, Ruan~\shortauthors~\cite{ruan2021dynamic}
%introduce a notion of approximation which we call {\em $\rho$-absolute-approximate}. 
Given a constant parameter $\rho \in (0, 1)$, 
%there are three relaxed cases of the similar neighbor definition:
the label of an edge $(u,v)$ is decided as follows:
\begin{enumerate}[leftmargin=*]
    \item if $\sigma(u, v) > \epsilon + \rho$, 
$(u,v)$ must be labelled as similar;
%$u$ and $v$ must be considered as similar neighbors; 
    \item if $\sigma(u, v) < \epsilon - \rho$, 
$(u,v)$ must not be labelled as similar;
%$u$ and $v$ must be considered as dissimilar neighbors. 
\item otherwise, i.e., $\epsilon - \rho \leq \sigma(u, v) \leq \epsilon + \rho$, 
the label of $(u,v)$ can be either similar or dissimilar.
%$u$ and $v$ could be considered as either similar or dissimilar neighbors;
\end{enumerate}
Once 
the edge labels are decided according to the above $\rho$-absolute-approximation,
all the other definitions introduced in Section~\ref{sec:prob} immediately follow.

It has been shown~\cite{} that clustering result under the notion of $\rho$-absolute-approximation provides
a ``sandwich'' guarantee on the result quality comparing the exact clustering result with the same parameters $\eps$ and $\mu$. 

\vspace{1mm}
\noindent
{\bf The Implementation of {\em EdgeSimStr}.}
BOTBIN maintains a {\em bottom-$k$ signature} for each vertex $u \in V$ for some integer parameter $k$.
Specifically, it first generates and stores a fixed random permutation $\pi$ on all the vertices in $V$.
For each vertex $u\in V$, 
if $d_u \geq k$, then the {\em signature} of $u$, denoted by $s(u)$, is the set of the $k$ smallest neighbors in $N[u]$ according to 
the permutation order $\pi$; 
otherwise, $s(u) = N[u]$.
With the bottom-$k$ signatures, an $\rho$-absolute-approximate Jaccard similarity, denoted by $\tilde{\sigma}(u,v)$, between any two vertices $u$ and $v$ is computed as 
$\tilde{\sigma}(u,v) = \frac{|s(u) \cap s(v) \cap s(\{u,v\})|}{k}$, where $s(\{u,v\})$ is the $k$ smallest vertices in $s(u) \cup s(v)$ according to the permutation $\pi$; if $|s(u) \cup s(v)| < k$, then $s(\{u,v\}) = s(u) \cup s(v)$.

\begin{itemize}[leftmargin = *]
\item update($(u,v)$, $op$): update the signatures $s(u)$ and $s(v)$ with respect to the update of $(u,v)$ accordingly; this can be achieved in $O(\log n)$ time with a sorted list of $N[u]$ by the permutation $\pi$. 
Thus, $\costeu \in O(\log n)$.
 
\item find($(u,v)$, $op$): if the signature $s(u)$ is changed due to this given update of $(u,v)$, add all the edges incident on $u$ to $F$; and perform the same symmetrically for $v$.
As a result, either $s(u)$ or $s(v)$ changes, then $\costef \in O(d_{\max})$; otherwise, $\costef \in O(1)$.

\item cal-sim($(x, y)$): return $\tilde{\sigma}(x,y)$ as the similarity of $x$ and $y$. Thus, this can be done in $O(k)$ time.
\end{itemize}

\vspace{1mm}
\noindent
{\bf The Implementation of {\em CoreFindStr}.}
BOTBIN implements {\em CoreFindStr} as an array, called {\em $\Delta$-table} and denoted by $T_{\Delta}$, of $\lceil \frac{1}{\Delta} \rceil$ sorted list of vertices, where $0 < \Delta < 1$ is a {\em constant}. 
Specifically, 
the parameter $\Delta$ partitions value range of $\eps$ into $\lceil \frac{1}{\Delta} \rceil$ intervals, where the $i^\text{th}$ interval is $(i \cdot \Delta, (i + 1) \cdot \Delta]$ for $i = 0, \cdots, \lceil \frac{1}{\Delta}\rceil-1$.
$T_{\Delta}[i]$ 
is a sorted list of all vertices $u \in V$ in {\em non-increasing} order by
$\mu_{u,i}$, where $\mu_{u,i}$ is 
 the number of neighbors of $u$ whose similarities to $u$ are at least $i \cdot \Delta$.
\begin{itemize}[leftmargin = *]
\item find-core($\eps$, $\mu$): identify $i^* = \lfloor \eps / \Delta \rfloor$; retrieve all the core vertices by scanning and reporting the vertices in the sorted list $T_{\Delta}[i^*]$ until the first vertex $x$ such  
that $\mu_{x,i^*} > \mu$ or the entire list has been retrieved.
The running time of this function $\costcf \in O(|\Vc| + 1)$.

\item update($x$): maintain the $\lceil \frac{1}{\Delta} \rceil$ sorted lists in $T_{\Delta}$ for $x$. 
This takes $\costcu \in O(\lceil \frac{1}{\Delta} \rceil \cdot \log n) = O(\log n)$ time.

\end{itemize}

\vspace{1mm}
\noindent
{\bf Theoretical Analysis.}
Zhang~\shortauthors~\cite{} showed that by setting $k \in O(\frac{1}{\rho^2} \cdot \log (n\cdot M) ) = O(\log (n \cdot M))$ and $\Delta = \frac{1}{2}\rho$, BOTBIN guarantees to return a valid $\rho$-absolute-approximate clustering result with high probability at least $1 - \frac{1}{n}$ for every query  and this holds for up to $M$ updates.   

\noindent
\underline{\em Query Running Time.} Since $\costcf$ in bounded by $O(|\Vc| +1)$, the running time of each query is bounded by $O(m_{cr})$. 

\noindent
\underline{\em Per-Update Running Time.}
Substitute the running time cost of each function in the above implementation to Expression~\eqref{eq:query-bound},
the per-update running time of BOTBIN is thus bounded by $O(|F| \cdot \log (n\cdot M)) \subseteq O(d_{\max} \cdot \log (n\cdot M))$.
While this per-update bound is still prohibitive, Zhang~\shortauthors proved that, as long as the $M$ updates happen {\em uniformly at random} in the neighborhood of each vertex,
then the signature of a vertex $u$ changes with probability $\frac{k}{d_u}$.
Therefore, the expected size of the ``invalid'' affected edge set $F$ is bounded by $O(\frac{k}{d_u} \cdot d_u) = O(\log (n\cdot M))$.
As a result, the expected per-update cost is bounded by $O(\log^2 (n\cdot M))$. 

\begin{comment}
\vspace{1mm}
\noindent
\underline{\em Space Consumption.} It can be verified that the space consumption of BOTBIN is bounded by $O(n + m)$ at all times.
\end{comment}

\begin{fact}
BOTBIN can return a valid $\rho$-absolute-approximate clustering result (under Jaccard similarity {\em only}) in $O(m_{cr})$ time with high probability at least $1 - \frac{1}{n}$ for any query, and this holds for up to $M$ updates.
Furthermore, it can handle each update in $O(d_{\max} \cdot \log (n\cdot M))$ time and the space consumption is bounded by $O(n + m)$ at all times. 

When the $M$ updates occur uniformly at random in the neighborhood of each vertex, then the per-update time is bounded by $O(\log^2 (n \cdot M))$ in {\em expectation}.  
\end{fact}

%\vspace{1mm}
\noindent
{\bf Remark.}
There are two main limitations of BOTBIN:
\begin{itemize}[leftmargin = *]
\item BOTBIN can handle Jaccard similarity only. 
%And it is still not clear that if it can support Cosine and Dice similarity measurements. 
However, in certain real-world applications~\cite{SCAN orginal paper}, Cosine and Dice similarities may be more preferable. 
%are important to real-world applications.  

\item The $O(\log^2 (n\cdot M))$ expected per-update bound of BOTBIN only holds for random updates. However, in many applications, the updates are not random, e.g., people tends to follow big names in social networks.  
Even worse, by repeatedly inserting and deleting certain {\em critical} edge which changes the signatures of its two end-vertices, BOTBIN has to pay $O(d_{\max}\cdot \log (n\cdot M))$ cost for each such update.


\end{itemize}



\begin{comment}

In addition to the sorted neighbor list for each vertex, GS*-index implements the two modules: {\em EdgeSimStr} and {\em CoreFindStr}, in the unified algorithm framework as follows:
\begin{itemize}[leftmargin = *]

\item {\em CoreFindStr}: The GS*-index implements the {\em CoreFindStr} module as a so-called {\em $\mu$-Table}, denoted by $T$,  which is essentially an array of $d_\max$ sorted lists.
%For each vertex $u\in V$, denote the $i^\text{th}$ largest similarity of $u$ to its neighbors by $\eps_{u, i}$, for integer $1 \leq i \leq d_u$. 
Specifially, for integer $1 \leq i \leq d_\max$, $T[i]$ stores a {\em sorted} list of all the vertices $u$ (with degrees $d_u \geq i$) in a {\em non-increasing} order by $\eps_{u, i}$, where $d_{\max}$ is the largest vertex degree in $G$ and  $\eps_{u,i}$ is   
the $i^\text{th}$ largest similarity of $u$ to its neighbors.
%by the similarity values $\eps_{u, i}$.
%the $i^\text{th}$ {\em largest} similarity to their neighbors. 
The rationale of the $\mu$-Table is that, 
for any given query parameters $\eps$ and $\mu$,
all the core vertices can be retrieved by scanning and reporting the vertices in the sorted list of $T[\mu]$ until the first vertex $u$ such that $\eps_{u, \mu} < \eps$ is met or the entire list has been retrieved.
\end{itemize}

\vspace{1mm}
\noindent
{\bf Answering Queries.}
For a query with parameters $\eps$ and $\mu$,
GS*-index first retrieves $\Vc$ by scanning $T[\mu]$ in $O(|\Vc|)$ time, and then, obtains $E_{cr}$ from the  
sorted neighbor lists of the core vertices. 
Finally, return the clustering result with the induced graph $G_{cr}$ of $E_{cr}$.
The query running time is clearly bounded by $O(|E_{cr}|)$.

\vspace{1mm}
\noindent
{\bf Handling Updates.}
For an update of edge $(u,v)$, 
GS*-index first compute $\sigma(u,v)$ and records the intersection size $I(u,v)$ of $N[u]$ and $N[v]$, if this update is an insertion.
Since GS*-index is an exact algorithm, 
all affected edges of this update of $(u,v)$ are considered ``invalid'', because  the degrees of $u$ and $v$ have been changed.
As a result, $F$ is the set of all these affected edges.
This implements Step 2 in update algorithm in the unified framework.
%
To implement Step 3, for each edge $(w_1,w_2) \in F$, GS*-index updates $I(w_1,w_2)$ and re-calculates $\sigma(w_1,w_2)$ with $I(w_1, w_2)$, $d_{w_1}$ and $d_{w_2}$. And then, it maintains the sorted neighbor lists of $N[w_1]$ and $N[w_2]$ accordingly.  
%
To implement Step 4, let $S$ be the set of all the end-vertices of the edges in $F$ plus $u$ and $v$;
for each vertex $w \in S$, GS*-index updates the sorted lists in $T[i]$ for $w$ accordingly, where $1 \leq i \leq d_w$.  

Moreover, it is not difficult to analyse that the overall running time for each update is bounded by $O(d^2_{\max} \log d_{\max}) \subseteq O(n^2 \log n)$, 
and the overall space consumption of GS*-index is bounded by $O(n + m)$ at all times.
\end{comment}

%\vspace{1mm}
%\noindent
%{\bf Analysis.}
%To analyse the running time for each update, first computation of $\sigma(u,v)$ takes $O(d_u + d_v) \subseteq O(d_\max)$ time.
%As there are $d_u + d_v$ edges in $F$, Step 2 takes $O(d_\max)$ time. 
%For Step 3, for each edge $(w_1, w_2) \in F$ takes $O(1)$ time to update $I(w_1, w_2)$ and re-calculate $\sigma(w_1, w_2)$, and $O(\log d_{\max})$ time to update the sorted neighbor lists of $w_1$ and $w_2$. Thus, the overall cost of Step 3 is bounded by $O((d_u + d_v) \cdot \log d_\max)$ time. 



\section{old version}


\subsection{SOTA for Dynamic Structural Clustering}
\label{subsec:rho}

We start with the Dynamic Structural Clustering (DynStrClu) problem, where the parameters $\eps$ and $\mu$ are pre-specified and fixed.
And we introduce the STOA algorithm, {\em DynELM}~\cite{ruan2021dynamic}, for solving this setting.
As we shall see in Section~\ref{sec:}, 
our proposed algorithm follows the same algorithm framework as that of {\em DynELM}, though the techniques we adopted are different.


\subsubsection{Dynamic Edge Label Maintenance (DynELM)}

As its name suggested, the main idea of {\em DynELM} is to maintain 
%the set $V_{\text{core}}$ of all the core vertices and 
the labels (either similar or dissimilar) for all the edges in $G$ under updates. 
To achieve this, for each vertex $u \in V$, {\em DynELM} maintains two sets of $u$'s neighbors: one set contains all $u$'s similar neighbors, and the other contains all its dissimilar neighbors.
Upon a query, i.e., a request to output the current clustering result, 
{\em DynELM} 
performs the following steps:
\begin{itemize}[leftmargin = *]
%\item  retrieve $V_{\text{core}}$, the set of all the core vertices;
\item for each vertex $u \in V$, if $u$ is a core vertex, then retrieve all its similar neighbors; the clustering result graph $G_{cr}$ is hence obtained; \jz{what's to compute in the next step then?}
\item  compute and return the clustering result with $G_{cr}$. 
\end{itemize}
It can be verified that the running time of the above query algorithm is bounded by $O(n + |E_{cr}|)$. 
To improve this bound to $O(|E_{cr}|)$, 
one can just  
further maintain a set $V_{\text{core}}$ recording all the current core vertices when the edge labels are maintained: if the label of an edge $(u,v)$ flips, check whether the core status of $u$ (resp., $v$) changes; if so, add or remove $u$ (resp., $v$) to/from $V_{\text{core}}$ accordingly.  
This maintenance can be performed in an extra $O(1)$ time, in addition to the edge label maintenance cost.
The main difficulty still lies in how to efficiently maintain the edge labels under updates to $G$. 

Unfortunately, 
maintaining the {\em exact} labels for the edges is costly. 
To see this, there are two technical challenges: 
\begin{itemize}[leftmargin = *]
\item Firstly, computing the similarity (i.e., label) for an edge $(u,v)$ inserted to $G$,
takes $\Omega(\min\{d_u, d_v\}) = \Omega(d)$ time, where $d_u$ and $d_v$ are the degrees of $u$ and $v$, respectively, and $d$ is the maximum degree of the vertices in $G$.
\item Secondly, for each insertion or deletion with respect to an edge $(u,v)$, the neighborhood $N[u]$ (resp., $N[v]$) changes, and hence, it could lead to a label change for every edge incident on $u$ (resp., $v$). As a result, the maintenance cost for the labels of those edges takes $\Omega(d_u + d_v) = \Omega(d)$ time in the worst case.  
\end{itemize}
Therefore, the cost to maintain exact edge labels is inevitably $\Omega(d) = \Omega(n)$ in the worst case. 

\vspace{1mm}
\noindent{\bf $\rho$-Absolute-Approximation.}
The overcome these challenges, Ruan~\shortauthors~\cite{ruan2021dynamic}
introduce a notion
of approximation which we call {\em $\rho$-absolute-approximate}. 
Given a constant parameter $\rho \in (0, 1)$, 
%there are three relaxed cases of the similar neighbor definition:
the label of an edge $(u,v)$ is decided by the following three cases:
\begin{enumerate}[leftmargin=*]
    \item if $\sigma(u, v) > \epsilon + \rho$, 
$(u,v)$ must be labelled as similar;
%$u$ and $v$ must be considered as similar neighbors; 
    \item if $\sigma(u, v) < \epsilon - \rho$, 
$(u,v)$ must not be labelled as similar;
%$u$ and $v$ must be considered as dissimilar neighbors. 
\item otherwise, i.e., $\epsilon - \rho \leq \sigma(u, v) \leq \epsilon + \rho$, 
the label of $(u,v)$ can be either similar or dissimilar.
%$u$ and $v$ could be considered as either similar or dissimilar neighbors;
\end{enumerate}
Once 
%the similar and dissimilar relationship between the vertices (i.e., 
the edge labels are decided according to the above $\rho$-absolute-approximation,
all the other definitions introduced in Section~\ref{sec:..} immediately follow.

\vspace{1mm}
\noindent{\bf Similarity Estimation.}
With the $\rho$-absolute-approximation,
{\em DynELM}  
adopts a sampling approach to compute, with high probability, an 
estimation $\hat{\sigma}(u,v)$ within a $\frac{1}{2}\rho$ absolute error to the {\em Jaccard Similarity} $\sigma(u,v)$. 
It has been shown that $\hat{\sigma}(u,v)$ can be computed in 
$O(\log^2 n)$ time.
An edge $(u,v)$ is labeled as similar if $\hat{\sigma}(u,v) \ge \epsilon$; otherwise, it is labeled as dissimilar.


\vspace{1mm}
\noindent{\bf Update Affordability.}
The $\rho$-absolute-approximation cannot avoid $\Omega(d)$ cost for the edge label flips.
This is because, for an update with edge $(u,v)$, it is still possible that all labels of the edges incident on $u$ flip. 
To see this, for example, \tocheck{in Figure~\ref{fig:clustering_exp}, when edge $(v_2, v_1)$ is deleted, the labels of $(v_2, v_5)$ and $(v_2,v_5)$ flips under the Jaccard Similarity with $\epsilon = 0.5$.}
Nonetheless, 
Ruan~\shortauthors~observe that once an edge $(u,v)$ is labelled with a $\frac{1}{2}\rho$-absolute approximate $\hat{\sigma}(u,v)$, 
the label can remain unchanged for a certain number of {\em  affecting updates} without violating the $\rho$-absolute-approximation.
Here, an affecting update of an edge $(u,v)$ is 
an update having  either $u$ or $v$ or both as its endpoint(s).
\begin{fact}[\cite{ruan2021dynamic}]
\label{fact:flip}
   For Jaccard Similarity,  consider an edge $(u, v)$ 
which is just labelled by a $\frac{1}{2}\rho$-absolute-approximate $\hat{\sigma}(u,v)$;
the label of $(u,v)$ can remain unchanged for at least $\ell = \lfloor \frac{1}{2}\rho\cdot\max(d_u, d_v)\rfloor$ affecting updates without violating the $\rho$-absolute-approximation.
%before its label changes from a similar edge to a dissimilar edge, and vice versa.
%T~\footnote{The $\rho-$approximation is defined as a relative error originally~\cite{ruan2021dynamic}, i.e., $(1 + \rho)\epsilon$. A follow-up study~\cite{zhang2022effective} defines it as an absolute error such that $\epsilon$ can be removed from $l$ as shown above - we follow this definition in our study.}
\end{fact}

\vspace{1mm}
\noindent{\bf The Algorithm Framework.} 
The key idea of {\em DynELM} is to re-compute $\hat{\sigma}(u,v)$ of an edge $(u,v)$ only when its update affordability runs out. 
%To accomplish that, the algorithm framework of {\em DynELM} consists of two main components: 
%(1) update affordability tracking, to track how many updates have affected an edge and its remaining affordability; (2) similarity estimation, to reduce the complexity of computing similarity score. With the labels of the edges, the steps of their algorithm regarding a graph update $(u,v)$ can be summarized below:
Specifically, given an update with edge $(u,v)$ to the graph $G$, {\em DynELM} works as follows:
\begin{itemize}[leftmargin=*]
    \item {\bf Step 1.} If the update is an insertion of $(u, v)$, estimate the similarity score $\hat{\sigma}(u,v)$; label $(u,v)$ as similar if $\hat{\sigma}(u,v) \geq \epsilon$; otherwise, label $(u,v)$ as dissimilar. 
If the update is a deletion of $(u, v)$, remove $(u,v)$ from $G$.
    \item \textbf{Step 2.} 
If any edge $(u,w)$ incident on $u$ runs out of its update affordability,  
re-compute $\hat{\sigma}(u,w)$ and label $(u,w)$ accordingly.
%For all the edges connected to $u$, if their affordability runs out, estimate the similarity score and set the label accordingly.
    \item \textbf{Step 3.} Perform \textbf{Step 2} symmetrically for $v$.
\end{itemize}

\vspace{1mm}
\noindent {\bf Update Affordability Tracking.} 
%In order to track when the update affordability of an edge runs out, 
{\em DynELM} creates a {\em Distributed Tracking} (DT)~\cite{cormode2011algorithms, huang2012randomized, keralapura2006communication} instance, for each edge $(u,v)\in E$, to 
track to exact moment when the update affordability of $(u,v)$ runs out.
The DT instances of all edges incident on $u$ (for each $u \in V$) are organized by a heap. 
%Ruan~\shortauthors~show that
%each such tracking can be achieved in $O(\log^2 n)$ amortized time. 
%Ruan~\shortauthors's algorithm simulates a \emph{Distributed Tracking} problem~\cite{cormode2011algorithms, huang2012randomized, keralapura2006communication} for update affordability tracking and organizes the DT instances in a heap, which achieves $O(\log^2 n)$ time complexity.

\vspace{1mm}
\noindent
{\bf Putting Everything Together.}
%Ruan~\shortauthors~show the following fact:
\begin{fact}[\cite{ruan2021dynamic}]
{\em DynELM} 
%correctly maintains the edge labels (under $\rho$-absolute-approximation) with high probability, 
supports each update in $O(\log^2 n)$ amortized time,
and returns a clustering result, satisfying the $\rho$-absolute-approximation with high probability, in $O(|E_{cr}|)$ time upon request. 
\end{fact}

\vspace{1mm}
\noindent
{\bf Limitations.}
{\em DynELM} supports Jaccard Similarity {\em only},
and does not support queries with parameters $\epsilon$ and $\mu$ given on the fly.


\subsection{SOTA for DynStrClu for All Parameters}

%\subsubsection{A Naive Algorithm}
\jz{Can we skip Section 2.2 and go straight into Section 2.3 and just present a solution framework for DynStrClu for All Parameters?}

\subsubsection{GS*-Index}
\input{figures/figure_scripts/indexing_example}
We now introduce the GS*-Index structure that groups the vertices by the possible $\mu$ inputs, which was first proposed by Wen \shortauthors~\cite{wen2017efficient}. The main idea is to calculate $\epsilon_{\mu, v}$ for all vertices and all possible $\mu$, where $\epsilon_{\mu, v}$ is the maximum $\epsilon$  for which vertex $v$ can have at least $\mu$ similar neighbors. For example, if $\epsilon_{3, v} = 0.5$, there are at least 3 vertices in $N[v]$ whose similarity scores are greater than or equal to $0.5$. The $\epsilon_{\mu, v}$ values of all vertices are grouped by $\mu$ and sorted based on $\epsilon_{\mu, v}$ in each group in descending order as shown in Figure~\ref{fig:gs_index}. 

A sorted linked list $NO[v]$ for each vertex is also maintained. This index structure can accelerate structural clustering query for any given $\mu$ and $\epsilon$ to $O(n_{cr} + m_{cr})$ time. When given a $\mu$ and a $\epsilon$, computing structural clustering only needs to locate the corresponding $\mu$ group and scan the elements in the group until $\epsilon > \epsilon_{\mu,v}$. All the scanned vertices except the last one are core vertices, and the sorted linked list $NO$ of each of these core vertices is then scanned to obtain their similar neighbors. 

The update cost for this index mainly comes from maintaining the sorting order in each $\mu$ group. When $\sigma(v, w)$ is changed, for the $\mu$ group that contains $w$, the corresponding $(\mu, \epsilon_{\mu, w})$ needs to be re-inserted. Each re-insertion takes $O(\log n)$ time, and in total the update takes $O(d^2\log n)$ time as there are $d_v$ vertices in $N[v]$, and there are $d_w$ groups containing $w$.

% Applying our \emph{RSCM} framework, $\sigma(u, v)$ is updated after $O(d_{max}(u,v))$ updates affecting $(u, v)$, and there are at most $d_v$ groups containing $v$ which makes the amortized time $O(d\log n + \log \frac{M}{p_f})$.

% \begin{lemma}
%     The $\mu$ table index takes $O(n+m)$ space.
% \end{lemma}

% \begin{proof}
%     Each vertex $u$ appears in at most $d_u$ groups. Thus, the total size of the $\mu$ tables is $\sum_{u \in V}d_u = 2m \in O(n+m)$.
% \end{proof}


\subsubsection{BOTBIN}
\label{subsec:eps-bucket}
Another index structure proposed by ~\citet{zhang2022effective} has a similar idea, but the vertices are grouped into constant number buckets to avoid $O(d^2\log n)$ update cost. The index schema also generates the $\mu, \epsilon$ pairs, while this time the maximum number of similar neighbors $\mu_{\epsilon_i-\epsilon_{i+1}}$ under each given $\epsilon$ is recorded, where $i$ is a bucket index. As $\epsilon$ is a real number with infinitely different values in its range $(0, 1)$, the range is divided into $\delta$ buckets, and for each bucket, the vertices are sorted by its $\mu_{\epsilon_i-\epsilon_{i+1}}$ value in descending order as shown in Figure~\ref{fig:botbin}. In this way, they only need to update the affected vertices in at most $\delta$ buckets, hence the complexity is reduced to $O(\frac{1}{\delta}d\log n) \subseteq O(d\log n)$. As they apply the bottom-$k$ hashing to estimate the Jaccard Similarity, \emph{with the assumption that the update is uniformly distributed}, the chance of an update to affect the $k$ elements is $\frac{k}{d}$. The estimated similarity requires re-computed only when the $k$ elements are changed. Therefore their algorithm can achieve an expected $O(\frac{k}{d}d\log n) \subseteq O(\log^2 n)$ under such assumption, where $k \in O(\log n)$.   

For the querying process, the bucket that covers the input $\epsilon$ is checked to obtain the core vertices, and then the vertices are scanned in order until a vertex with $\mu_{\epsilon_i-\epsilon_{i+1}} < \mu$ is found. The index update only needs to update at most $\frac{1}{\delta}$ buckets instead of $n$ groups, as in the $\mu$ table index. However, this comes at the expense of increasing the approximation error by $\delta$. When $\epsilon - \rho \leq \sigma(u, v) \leq \epsilon + \rho + \delta$, $u$ and $v$ may be considered either similar or dissimilar when finding the core vertices. This is because, in the worst case, when calculating $\mu_{\epsilon_i-\epsilon_{i+1}}$, if the estimated $\hat{\sigma}(u, v) = \epsilon_{i}$, it is still considered as similar when the input $\epsilon = \epsilon_{i+1}$, and $\epsilon_{i+1} - \epsilon_{i} = \delta$.

\jz{Too many detailed issues to understand the limitations of the existing solutions. How about we just describe a solution framework and proceed to talk about our algorithm design for each component? Later, we come back to spend a subsection to talk about how our solution differs from the SOTA? Or at the minimum, plot a solution framework figure to help highlight which parts we improve upon, like Zhifeng suggested.}



\begin{comment}
\section{old version}


% \junhao{following this logic flow: (i) define $\rho$-approxiation; (ii) mention that because of the approximation, we are now allowed to use approximate similarity and not have to check every affected edges for each update; (iii) introduce the algorithm framework}

% \junhao{you will need to first define (i) affected edges, and (ii) update affordability}

% \junhao{introduce DynELM in the way of an implementation of the algorithm framework, i.e., (i) how to estimate the similarity and (ii) how to ``track'' the update affordability for the edges. This also applies to our algorithm presentation in Section 4.}

To facilitate the illustration of our proposed method, we first review dynamic structural clustering~\cite{ruan2021dynamic} and the SOTA algorithm \emph{DynELM}~\cite{ruan2021dynamic}. 

\noindent\underline{$\rho$-approximation.} Ruan~\shortauthors~\cite{ruan2021dynamic} proposed a $\rho$-approximation to relax the definition of similar neighbors that enables efficient dynamic structural clustering, which we follow. 
Given a constant parameter $\rho \in (0, 1)$, there are three relaxed cases of the similar neighbor definition:
\begin{enumerate}[leftmargin=*]
    \item $\sigma(u, v) > \epsilon + \rho$: $u$ and $v$ must be considered as similar neighbors.
    \item $\epsilon - \rho \leq \sigma(u, v) \leq \epsilon + \rho$: $u$ and $v$ could be considered as either similar or non-similar neighbors.
    \item $\sigma(u, v) < \epsilon - \rho$: $u$ and $v$ must be considered as non-similar neighbors. 
\end{enumerate}
Under the $\rho$-approximation settings, they have defined:
\begin{itemize}[leftmargin=*]
    \item \emph{$(\epsilon, \rho)$-neighbor}: given an $\epsilon$ and a $\rho$, two vertices are $(\epsilon, \rho)$-neighbors when it satisfies the relaxed definition above.  
    \item \emph{$(\mu, \epsilon)$-core}: given an $\epsilon$ and an $\mu$, a vertex is a \emph{$(\mu, \epsilon)$-core} vertex if it has at least $\mu$ \emph{$(\epsilon, \rho)$-neighbors}.
\end{itemize} 
The clustering results are then decided based on $(\epsilon, \rho)$-neighbors and $(\mu, \epsilon)$-cores.

\noindent\underline{A crucial observation.} In dynamic scenarios, maintaining the exact edge labels is costly. For example, when an update $(u,v)$ comes, in the worst case, the labels for all $(u,w) | w \in N[u]$ can flip, which takes $\Omega(d)$. With the relaxed definition, they are now allowed to use approximate similarity estimation, denoted as $\hat{\sigma}(u,v)$, eliminating the need for re-computing the similarity of each edge when it is affected, as long as the similarity change is within the error bound. Ruan~\shortauthors~introduce the notion of ``update affordability", indicating the number of updates an edge can afford. To elucidate their algorithmic framework, we will first articulate the concept of affected edges and subsequently delve into the definition of update affordability.


\noindent \textbf{Affected edges}. When an update $(u,v)$ (either insertion or deletion) comes, the similarity score $\sigma(u, w)$ for $w \in N[u]$ may change \jz{$N[v]\cup N[u]$ could change too? \tocheck{yes, but it can be easily calculated when $|N[u]\cap N[w]$ is known}}. This is because $|N[u]\cap N[w]$ will change if $v$ is a neighbor of $w$.  Symmetrically, $\sigma(v, w) | w \in N[v]$ could change, too. Therefore, an update $(u,v)$ can affect $d_u + d_v$ edges, which is $O(n)$ in the worst case. We call the edges that are affected by an update affected edges. 

\noindent \textbf{Update affordability}. The cluster results are decided by \emph{$(\epsilon, \rho)$-neighbors} of each vertex. As long as the \emph{$(\epsilon, \rho)$-neighbor} relationship remains unchanged, the clustering results remain the same. When an edge is affected, it does not necessarily entail a change in the edge's label. In fact, Ruan~\shortauthors~have proved that:
\begin{fact}
\label{fact:flip}
    With a probability of at least $1 - p$, an edge $(u, v)$ can afford at least $l = \lfloor \frac{1}{2}\rho\cdot\max(d_u, d_v)\rfloor$ affecting updates before it changes from a similar edge to a dissimilar edge, and vice versa.~\footnote{The $\rho-$approximation is defined as a relative error originally~\cite{ruan2021dynamic}, i.e., $(1 + \rho)\epsilon$. A follow-up study~\cite{zhang2022effective} defines it as an absolute error such that $\epsilon$ can be removed from $l$ as shown above - we follow this definition in our study.}
\end{fact}

\noindent\underline{Algorithm Framework.} Their key idea is to re-compute the similarity score of an edge only when its update affordability runs out. To accomplish that, their algorithm framework consists of two main components: (1) update affordability tracking, to track how many updates have affected an edge and its remaining affordability; (2) similarity estimation, to reduce the complexity of computing similarity score. With the labels of the edges, the steps of their algorithm regarding a graph update $(u,v)$ can be summarized below:
\begin{itemize}[leftmargin=*]
    \item \textbf{Step 1.} If $(u, v)$ is an insertion, estimate the similarity score $\hat{\sigma}(u,v)$; set the label of $(u,v)$ as similar if $\hat{\sigma}(u,v) < \epsilon$, otherwise set the label dissimilar. If $(u, v)$ is a deletion, remove $(u,v)$'s label.
    \item \textbf{Step 2.} For all the edges connected to $u$, if their affordability runs out, estimate the similarity score and set the label accordingly.
    \item \textbf{Step 3.} Perform \textbf{Step 2} symmetrically for $v$.
\end{itemize}

\noindent\underline{Similarity Estimation.} Ruan~\shortauthors~developed a sampling method that accelerates the similarity computation from $O(n)$ to $O(\log n \log \frac{M}{p_f})$, where $O(\log \frac{M}{p_f})$ is the sampling cost for $M$ updates and $O(\log n )$ comes from an implementation of a binary search tree (BST). Their method also guarantees a good error bound of the similarity estimation with a low failure probability $p_f$, leading to high-quality clustering results. If we replace the \emph{BST} implementation with hashing, the sampling method can achieve $O(\log \frac{M}{p_f})$ expected cost.

\noindent\underline{Update affordability tracking.} Ruan~\shortauthors's algorithm simulates a \emph{Distributed Tracking} problem~\cite{cormode2011algorithms, huang2012randomized, keralapura2006communication} for update affordability tracking and organizes the DT instances in a heap, which achieves $O(\log^2 n)$ time complexity.

\end{comment}

% \noindent\textbf{Distributed tracking.} DT~\cite{cormode2011algorithms, huang2012randomized, keralapura2006communication} considers a distributed environment where there are $h$ participants and a coordinator $q$. There is a communication channel between each participant and the coordinator, while the participants cannot communicate with each other. Each participant has a counter $c_i$ initialized to 0, and at each time stamp, at most one of these counters can increase by 1. Given a threshold $\tau > 0$, $q$ must report ``maturity'' when $\sum^h_{i=1}c_i = \tau$. The optimization goal is to minimize the messages received and sent by $q$. 

% Tracking the number of times an edge is affected can be simulated as a DT problem as shown in Figure~\ref{fig:dt_framework}. A DT instance, $DT(u,v)$, is created for each edge $(u, v)$ that has a coordinator $q_{u,v}$ and 2 participants, $c_{u, v}$ and $c_{v, u}$ associated to vertices $u$ and $v$, respectively. If we only consider this single DT instance, when a graph update $(u, w)$ comes, $c_{u, v}$ is increased by 1, which indicates another update has just affected $(u, v)$. In this case, $\tau$ is set to the threshold when we need to re-compute $\sigma(u,v)$, which is $l + 1$ (Fact~\ref{fact:flip}). Therefore, as long as $q_{u,v}$ reports mature ($c_{u, v} + c_{v, u} = l + 1$), we re-compute $\sigma(u,v)$. 

% Tracking the number of times an edge is affected can be simulated as a DT problem where each edge is associated with a DT instance that reports ``maturity'' when the edge needs to be re-labelled. The DT problem is a well studied problem and can be solved in $O(h\log\frac{\tau}{h})$~\cite{huang2012randomized}. Applied to update affordability tracking, it can then be solved in $O(\log n)$ time as $h = 2$ and $\tau = \lfloor \frac{1}{2}\rho\cdot\max(d_u, d_v)\rfloor \in O(n)$. 

% The DT problem only considers the cost of communication, however, in this simulation, the cost of increasing the counters cannot be ignored. Each graph update could affect up to $d$ vertices, and it takes $O(n)$ time if we increase all the counters associated with them by 1. Ruan~\shortauthors~\cite{ruan2021dynamic} used shared counters and a heap to organize the DT instances to avoid this cost. The heap operation introduces an overhead cost $O(\log n)$, hence the total cost is $O(\log^2 n)$. 

% \noindent\underline{Handling shared counters.} \jz{Quite brief and not particularly how it works.} \tocheck{Might not be easy to describe how this works without describing the DT algorithm in~\cite{huang2012randomized}} Their algorithm is based on the DT algorithm proposed in~\cite{huang2012randomized} which asks the participants to report in rounds. For a graph update, instead of increasing all the counters associated with the affected edges, they only increase one counter shared by all DT instances.
% Specifically, for each vertex $u$, a common counter $s_u$ is shared by all $DT(u, v)$ where $v \in N[u] - {u}$, and we increase $s_u$ by 1 when $u$ is included by an update. Additionally, $\hat{c}_u{(u,v)}$ is used that does not track the exact affected number, but the moment it needs to report, i.e., when $s_u + 1 = \hat{c}_u{(u,v)}$. A min-heap is applied to organize the counter status for each DT instance with $\hat{c}$ as a key. With the min-heap, we can track the participants that are closest to being triggered to report and temporarily ignore the rest. 
% In this way, they can track the update affordability in $O(\log^2 n)$ cost consisting of $O(\log n)$ for DT and $O(\log n)$ for heap operations, e.g. element insertion and deletion.

% \begin{figure}
% \centering
% \includegraphics[width=0.4\textwidth]{figures/dt_framework.pdf}
% \caption{DT framework}
% \label{fig:dt_framework}
% \end{figure} 

%To generate such an index schema, it is necessary to compute the similarity scores for all pairs, which takes $O(md)$ time, where $d$ is the maximum degree. With the similarity scores, it takes $O(\log d_v)$ time to insert each vertex in $N[v]$ to get $NO[v]$. The total time complexity is $O(\sum_{v \in V} \log d_v) = O(m\log n)$, as $2m = \sum_{v \in V} d_v$. After that, $(\mu, \epsilon_{\mu, v})$ can be computed in $O(m \log n)$ by inserting each element of $NO[v]$ into each group, as each vertex can only appear $d_v$ times, and in the worst case, each $\mu$ group will have $n$ node.  

% \subsection{Limitations of SOTA Methods}
% For DynELM~\cite{ruan2021dynamic},   the tracking of update affordability through their DT-based approach has a time complexity of $O(\log^2 n)$. The key idea of the DT framework is to only re-compute the similarity after it has been affected $l$ times. However, this can be resource-intensive and pose a bottleneck for their algorithm. 
%tracking the number of affected times and reporting right at the $l^{th}$ affecting updates could be costly and become the bottleneck of their algorithm. 
% Under their problem formulation, In their problem formulation, predetermined values of $\epsilon$ and $\mu$ are required, preventing on-the-fly parameter support. 

% BOTBIN~\cite{zhang2022effective} improves the index schema maintenance costs using hashing and bucketing methods. %Nevertheless, it assumes a uniform update distribution for its complexity claim due to the hashing technique. 
% According to its claim, when an update $(u, w)$ occurs, BOTBIN has a probability of $\frac{k}{d_u}$  to alter the bottom-$k$ result of $N[u]$ and to re-compute the similarity between $u$ and its neighbors, resulting in lower average time complexity. However, this claim is true only when the update is uniformly distributed. In scenarios where consecutive insertions and deletions affect the bottom-$k$ result of a vertex, the algorithm may need to recalculate similarity $d$ times for each update, undermining the validity of the probability claim and the average complexity assertion. Additionally, due to the pre-permutation of vertices for hashing, BOTBIN encounters challenges in handling vertex insertions. 
%In addition, due to the permutation of each vertex in advance for hashing purposes, it is not trivial for BOTBIN to handle vertex insertions.

% Last, neither DynELM nor BOTBIN provide insight into the application of their methods when employing cosine similarity as the similarity measure.
%Further, neither DynELM nor BOTBIN discuss how to apply their methods when using cosine similarity as the similarity measure.




==> tables/cos_quality.tex <==
\begin{table}[ht]
\caption{Clustering quality results under Cosine similarity}
\vspace{-4mm}
\begin{small}
\begin{tabular}{l|c|c}
\hline
Datasets         & ARI $\uparrow$   & MLR $\downarrow$ \\ \hline
\texttt{soc-Slashdot0811} & 0.9900 & 0.10\%        \\ \hline
\texttt{web-NotreDame}    & 0.9863 & 0.15\%        \\ \hline
\texttt{web-Google}       & 0.9599 & 0.29\%        \\ \hline
\texttt{wiki-topcats}     & 0.9700 & 0.07\%        \\ \hline
\texttt{soc-Pokec}        & 0.9609 & 0.23\%        \\ \hline
\texttt{as-skitter}       & 0.9806 & 0.28\%        \\ \hline
\texttt{wiki-Talk}        & 0.9672 & 0.53\%        \\ \hline
\texttt{Orkut}            & 0.9673 & 0.14\%        \\ \hline
soc-LiveJournal1          & 0.9843 & 0.18\%        \\ \hline
\end{tabular}
\end{small}
\label{tab:cos_qua}
\vspace{-5mm}
\end{table}

==> tables/quality.tex <==
\begin{table}
\caption{Clustering quality results}
\vspace{-4mm}
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{l|cccc|cccc}
\hline
                 & \multicolumn{4}{c|}{$\rho = 0.02$}                                                                                & \multicolumn{4}{c}{$\rho = 0.1$}                                                                                  \\ \cline{2-9} 
                 & \multicolumn{2}{c|}{BOTBIN}                                      & \multicolumn{2}{c|}{\algo}                  & \multicolumn{2}{c|}{BOTBIN}                                      & \multicolumn{2}{c}{\algo}                   \\ \cline{2-9} 
                 & \multicolumn{1}{c|}{ARI $\uparrow$}    & \multicolumn{1}{c|}{MLR $\downarrow$} & \multicolumn{1}{c|}{ARI $\uparrow$}    & MLR $\downarrow$ & \multicolumn{1}{c|}{ARI $\uparrow$}    & \multicolumn{1}{c|}{MLR $\downarrow$} & \multicolumn{1}{c|}{ARI $\uparrow$}    & MLR $\downarrow$ \\ \hline
soc-Slashdot0811 & \multicolumn{1}{c|}{\textbf{0.9967}} & \multicolumn{1}{c|}{0.02\%}        & \multicolumn{1}{c|}{0.9963} & \textbf{0.01\%}        & \multicolumn{1}{c|}{0.9709} & \multicolumn{1}{c|}{1.60\%}        & \multicolumn{1}{c|}{\textbf{0.9718}} & \textbf{1.54\%}        \\ \hline
web-NotreDame    & \multicolumn{1}{c|}{0.9994} & \multicolumn{1}{c|}{\textbf{0.13\%}}        & \multicolumn{1}{c|}{\textbf{0.9997}} & \textbf{0.13\%}        & \multicolumn{1}{c|}{\textbf{0.9632}} & \multicolumn{1}{c|}{4.51\%}        & \multicolumn{1}{c|}{0.9627} & \textbf{4.43\%}        \\ \hline
web-Google       & \multicolumn{1}{c|}{\textbf{0.9991}} & \multicolumn{1}{c|}{\textbf{0.14\%}}        & \multicolumn{1}{c|}{0.9988} & \textbf{0.14\% }       & \multicolumn{1}{c|}{0.9695} & \multicolumn{1}{c|}{5.52\%}        & \multicolumn{1}{c|}{\textbf{0.9708}} & \textbf{5.45\% }       \\ \hline
wiki-topcats     & \multicolumn{1}{c|}{0.9990} & \multicolumn{1}{c|}{\textbf{0.06\%}}        & \multicolumn{1}{c|}{\textbf{0.9999}} & \textbf{0.06\%}        & \multicolumn{1}{c|}{\textbf{0.9896}} & \multicolumn{1}{c|}{\textbf{0.86\%}}        & \multicolumn{1}{c|}{0.9890} & 0.91\%        \\ \hline
soc-Pokec        & \multicolumn{1}{c|}{0.9957} & \multicolumn{1}{c|}{0.18\%}        & \multicolumn{1}{c|}{\textbf{0.9962}} & \textbf{0.17\%}        & \multicolumn{1}{c|}{0.9676} & \multicolumn{1}{c|}{\textbf{5.32\%}}        & \multicolumn{1}{c|}{\textbf{0.9682}} & 5.24\%        \\ \hline
as-skitter       & \multicolumn{1}{c|}{0.9995} & \multicolumn{1}{c|}{\textbf{0.19\%}}        & \multicolumn{1}{c|}{\textbf{0.9996}} & \textbf{0.19\%}        & \multicolumn{1}{c|}{0.9826} & \multicolumn{1}{c|}{6.38\%}        & \multicolumn{1}{c|}{\textbf{0.9841}} & \textbf{6.36\%}       \\ \hline
wiki-Talk        & \multicolumn{1}{c|}{0.9987} & \multicolumn{1}{c|}{0.45\%}        & \multicolumn{1}{c|}{\textbf{0.9991}} & \textbf{0.45\%}        & \multicolumn{1}{c|}{0.9716} & \multicolumn{1}{c|}{\textbf{7.29\%}}        & \multicolumn{1}{c|}{\textbf{0.9725}} & \textbf{7.29\%}        \\ \hline
Orkut            & \multicolumn{1}{c|}{0.9946} & \multicolumn{1}{c|}{0.12\%}        & \multicolumn{1}{c|}{\textbf{0.9954}} & \textbf{0.11\%}        & \multicolumn{1}{c|}{0.9548} & \multicolumn{1}{c|}{\textbf{4.38\%}}        & \multicolumn{1}{c|}{\textbf{0.9554}} & 4.43\%        \\ \hline
soc-LiveJournal1 & \multicolumn{1}{c|}{\textbf{0.9998}} & \multicolumn{1}{c|}{\textbf{0.12\%}}        & \multicolumn{1}{c|}{\textbf{0.9998}} & \textbf{0.12\%}        & \multicolumn{1}{c|}{0.9975} & \multicolumn{1}{c|}{4.56\%}        & \multicolumn{1}{c|}{\textbf{0.9995}} & \textbf{4.54\%}        \\ \hline
\end{tabular}
}
\label{tab:quality}
\end{table}

==> tables/related_work.tex <==
\begin{table}[t]
    \centering
        \caption{Related Works and Their Focuses}
    \label{tab:rw_tf}
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{l|c|c}
    \toprule
        Main focus& Related works & SOTA\\\hline
        \multirow{2}{*}{Static graph} &  SCAN~\cite{xu2007scan}, SCAN$++$~\cite{shiokawa2015scan++}, & \multirow{2}{*}{pSCAN} \\ & LinkSCAN*~\cite{lim2014linkscan}, pSCAN~\cite{chang2017mathsf} &\\\hline
        Dynamic graph & DynELM~\cite{ruan2021dynamic}, BOTBIN~\cite{zhang2022effective} & DynELM, BOTBIN\\\hline
        Index schema & BOTBIN~\cite{zhang2022effective}, GS*-Index~\cite{wen2017efficient} & BOTBIN \\\bottomrule
    \end{tabular}

\end{table}

==> tables/symbols.tex <==
\begin{table}[ht]
\setlength{\tabcolsep}{2pt}
  \caption{Frequently Used Symbols}
  \label{tab:freq}
  \begin{tabular}{cl}
    \toprule
    Notation & Description\\
    \midrule
    $n$ & $|V|$, the vertex set size\\
    $m$ & $|E|$, the edge set size\\
    $n_{cr}$ &  the vertex set size of structural cluster results\\
    $m_{cr}$ &  the edge set size of structural clusters results \\
    $d_u$ & the degree of vertex $u$\\
    $d$ & the maximum degree of any vertex in $V$\\
    $p_f$ & failure rate for similarity estimation\\
    $M$ & number of graph updates\\
    $N[u]$ & the neighborhood of $u$\\%, $N[u] = \{v \in V | (u,v) \in E\} \cup \{u\}$\\
    $NO[u]$ & the neighborhood of $u$ sorted by  $\sigma(u,v)$, $v \in N[u]$\\
    

  \bottomrule
\end{tabular}
\end{table}
